On testing pseudorandom generators via statistical tests based on the arcsine law

Testing the quality of pseudorandom number generators is an important issue. Security requirements become more and more demanding, weaknesses in this matter are simply not acceptable. There is a need for an in-depth analysis of statistical tests -- one has to be sure that rejecting/accepting a generator as good is not a result of errors in computations or approximations. In this paper we propose a second level statistical test based on the arcsine law for random walks. We provide a Berry-Essen type inequality for approximating the arcsine distribution, what allows us to perform a detailed error analysis of the proposed test.

==> sections/arcsine_tester.tex <==
In this Section we will show how to exploit the theoretical properties of random walks discussed in preceding sections
to design a practical routine for testing PRNGs. We briefly describe the approach based on 
the arcsine law which we employ
in experiments presented in Section \ref{sec:experiments}. 
%For the sake of completeness we will also recall some basic
%facts about the method of evaluating PRNGs presented in \cite{Wang2015}. 
Finally, we will perform the analysis
of approximation errors that occur in our testing procedure.

\subsection{The arcsine law based testing}
\label{subsec:arcsineTests}

  

The general idea of tests is the following: take a sequence of bits 
generated by PRNG (treat them as $-1$ and $+1$)
and compare the empirical distribution of 
\begin{equation*}
 \Sasin{n} = \frac{1}{n} \sum_{k=1}^n D_k \in[0,1]
\end{equation*}
(a fraction of time instants at which ones prevail zeros)
with its theoretical distribution assuming truly random numbers.
In terms of hypothesis testing: 
given the null hypothesis $\mathcal{H}_0$ that the sequence was randomly generated
(vs. $\mathcal{H}_A$: that the sequence was not randomly 
generated) 
the distribution of $\Sasin{n}$
% PRNG produced really
% 
% we will compare it to Arcsine Law given in Theorem \ref{twr:arcsine}. 
%For given $X_1,\ldots, X_n$ let
%\begin{equation}
%D_k = \mathbbm{1}\left(S_k > 0 \vee S_{k-1}>0 \right), k=1,2,\ldots,n.
%\end{equation}
%$D_k$ is equal to 1 if in $k$-th step number of ones prevails number of zeros
%(\textcolor{red}{traktując remisy tak jak w paragrafie \ref{sec:asin}}) and 0 otherwise.
%Let us define 
 follows the arcsine law (Theorem \ref{twr:arcsine}),
\ie we can conclude that  \textsl{for large } $n$ we have 
\begin{equation}\label{eq:prob_sasin}
%\begin{split}
% \label{eq:prob_sasin}
%  \Pro{\Sasin{n} \in (a,b)} &\approx \frac{1}{\pi} \int_a^b \frac{dt}{\sqrt{t(1-t)}}\\
%  &= \frac{2}{\pi}\arcsin(\sqrt{b}) - \frac{2}{\pi}\arcsin(\sqrt{a}).
%\end{split}
\Pro{\Sasin{n} \in (a,b)} \approx \frac{1}{\pi} \int_a^b \frac{dt}{\sqrt{t(1-t)}} = \frac{2}{\pi}\arcsin(\sqrt{b}) - \frac{2}{\pi}\arcsin(\sqrt{a}).
\end{equation}
(we will be more specific on ``$\approx$'' in Section \ref{sec:err_analysis}).
We follow the \textsl{second level} testing approach \cite{PareschiRS07}, \cite{Pareschi2007}, \ie we take into account several results from the same test over 
different sequences. To test a PRNG we generate $m$ sequences of length $n$ each. 
We thus obtain  $m$ realizations of a variable $\Sasin{n}$, the $j$-th 
replication is denoted by $\Sasin{{n,j}}$. We fix some partition of  [0,1]
and count the number of realizations of $\Sasin{n}$ which 
are in a given interval. In our tests we will use  $(s+1)$ 
element partition $\mathcal{P}^{asin}_s = \{ P^{asin}_1,   \ldots, P^{asin}_{s+1}\}$, 
where
\begin{equation*}
\begin{split}
  P^{asin}_1 &= \left[0, \frac{1}{2s}\right),\\
  P^{asin}_i &= \left[\frac{2i-3}{2s}, \frac{2i-1}{2s} \right),\ \ \ 2 \leq i \leq s,\\
  P^{asin}_{s+1} &= \left[1- \frac{1}{2s},1\right].
\end{split}
\end{equation*}
Now we define  measures $\mu^{asin}_n , \nu^{asin}_n $,
 $E_i$ 
 (the expected number of observations within $P^{asin}_i$) and 
 $O_i$ (the number of observations within $P^{asin}_i$):
 for $1 \leq i \leq s+1$,
\begin{align*}
\mu^{asin}_n \left( P^{asin}_i \right) & =  \Pro{\Sasin{n} \in P^{asin}_i}, \quad E_i=m \cdot \mu_n^{asin}(P_i^{asin}),\\ 
%\label{eq:mu_asin} 
\nu^{asin}_n \left( P^{asin}_i \right) &= \frac{|\{ j:\ \Sasin{{n,j}} \in  P^{asin}_i, 1 \leq j \leq m\}|}{m},
 \quad O_i=m \cdot \nu_n^{asin}(P_i^{asin}). 
 %\label{eq:emp_asin}
\end{align*}
We perform Pearson's goodness-of-fit test, which uses the following 
test statistic:
\begin{equation*}
\label{eq:chi_asin2}
 T^{asin} = \sum_{i=1}^{s+1} \frac{(O_i - E_i)^2}{E_i}
 = m \cdot\sum_{A\in \mathcal{P}^{asin}_s} {(\mu^{asin}_n(A) -\nu^{asin}_n(A))^2\over 
 \mu^{asin}_n(A)}.
\end{equation*}
Under the null hypothesis, $T^{asin}$ 
has approximately $\chi^2(s)$ distribution.  
We calculate the corresponding $p$-value 
$$p_{\chi^2} = \Pro{X>T^{asin}},$$
where $X$ has $\chi^2(s)$ distribution. 
Large values of $T^{asin}$ -- and thus small values of $p_{\chi^2}$ -- mean 
a given  PRNG is not good. 
Typically, we reject $\mathcal{H}_0$ (\ie we consider the 
test \textsl{failed}) if $p_{\chi^s}<\alpha,$ 
where $\alpha$ is a prescribed \textsl{level of significance}
(we will use typical $\alpha=0.01$).
Note that the probability of rejecting 
$\mathcal{H}_0$  when the sequence is generated by a perfect random 
generator (so-called \textsl{Type I error}) is $\alpha$.
\par 
Another approach is based on a \textsl{statistical distance 
based testing}, the approach was presented in \cite{Wang2015}.
We consider the statistic 
\begin{equation*}
\label{eq:dtv}
 d_{tv}^{asin} =  {1\over 2} \sum_{A\in \mathcal{P}^{asin}_s} 
 |\mu_n(A) -\nu_n(A)|\in[0,1],
\end{equation*}
\ie a total variation distance between the theoretical 
distribution $\mu^{asin}_n$ and the empirical 
distribution $\nu^{asin}_n $. Similarly, large values of 
$d_{tv}^{asin}$ indicate that a given  PRNG is not good. 
Concerning \textsl{Type I error} we will make use 
of the following lemma (see Lemma 3 in \cite{devroye1983}
or its reformulation, Lemma 1 in \cite{Berend2012}).
\begin{lem}\label{lem:devroy}
 Assume $\mathcal{H}_0$ and consider partition $\mathcal{P}_s^{asin}$, then  for all $\varepsilon \geq \sqrt{20 (s+1)/m} $ we have 
 $$\Pro{2d_{tv}^{asin} > \varepsilon} \leq 3 exp\left( -{m\varepsilon^2\over 25}\right).$$
\end{lem}



\medskip\par 
% 
% \pl{ASDF}
% and 
% 
% 
% % 
% % \begin{equation}
% % \label{eq:mu_asin}
% %  \mu^{asin}_n \left( P^{asin}_i \right) = P{\Sasin{n} \in P^{asin}_i}, 
% % \end{equation}
% % \begin{equation}
% %  \label{eq:emp_asin}
% %  \nu^{asin}_n \left( P^{asin}_i \right) = \frac{|\{ j:\ \Sasin{{n,j}} \in  P^{asin}_i, 1 \leq j \leq m\}|}{m}.
% % \end{equation}
% \noindent
% Measure $\mu^{asin}_n$ corresponds to the theoretical distribution and can 
% be approximately
% calculated by (\ref{eq:prob_sasin}), whereas 
% $\nu^{asin}_n$ represents empirical distribution obtained from tests.
% We will measure the distance  between these measures either using \textsl{total variation} or \textsl{separation} distance
%  defined for partition $\mathcal{P}$ as follows:
% %  
% % 
% % \textcolor{red}{ZMIENIC: If the PRNG is ``good'' then the measures should be close one to each other, what we will measure in various of ways.}
% % 
% % First, we will calculate \textsl{total variation} and \textsl{separation} distances defined for partition $\mathcal{P}$ as follows:
% \begin{align}
%  \label{eq:dtv_old}
%  d^{tv}_\mathcal{P}(\mu, \nu) &= \frac{1}{2} \sum_{A \in \mathcal{P}} |\mu(A) - \nu(A)|
%     %= \sum_{\substack{A \in \mathcal{P},\\ \mu(A) >\nu(A)}} \Big(\mu(A) - \nu(A)\Big),
%     ,\\
%  \label{eq:sep} 
% d^{sep}_\mathcal{P}(\mu, \nu) &= \max_{A \in \mathcal{P}}\left(1 - \frac{\mu(A)}{\nu(A)}\right).
% \end{align}
% Another approach is based on hypothesis testing. Using statistical terminology $\Sasin{{n,j}}$ will be called observations.
% Null hypothesis is that observations have distribution $\mu^{asin}_n$ , \ie that PRNG produces random bits.
% Define
% \begin{equation*}
%  O_i = |\{ j:\ \Sasin{{n,j}} \in  P^{asin}_i, 1 \leq j \leq m\}|,\ \ \ 0 \leq i \leq s+1,
% \end{equation*}
% the number of observations within $P^{asin}_i$ interval. Let $E_i$ denote expected number of observations within this interval,
% \ie $E_i=m\cdot\Pro{\Sasin{n}\in P^{asin}_i}$ (what is calculated from (\ref{eq:prob_sasin})). Assuming null hypothesis
% the statistic
% 

Summarizing, for a given PRNG we generate $m$ sequences of length $n$ each. 
Then we choose $s$ (and thus a partition $\mathcal{P}^{asin}_s$),
calculate $d^{asin}_{tv}$
 and $T^{asin}$ together with its $p_{\chi^2}$-value. 
We specify thresholds for $p_{\chi^2}$-value   and 
$d^{asin}_{tv}$ indicating if the test \textsl{failed} or not 
(details in Section \ref{sec:experiments}). We denote 
the described procedure as ASIN test.


\pl{TO DO: uwaga, ze to co robimy to dokladnie to samo co
w second-level testing, tzn., najpierw p-wartosci, a potem 
test jednostajnosci}

\smallskip\par Note that the described procedure is equivalent 
to the following one: calculate $p$-value  for $j$-th realization 
of $S_n^{asin}, j=1,\ldots,m$ directly from (\ref{eq:prob_sasin}), and then 
test if the distribution of these $p$-values is uniform. 
We stated it in the form presented in \cite{Wang2015}.
\textcolor{red}{UWAGA: napisalem tak, ale to do sprawdzenia!!!!}.
We could also calculate just one $p$-value of the statistic $S_{n'}^{asin}$ 
for longer sequence (say, for $n'=n\cdot m$) -- \ie perform a  \textsl{first level}
test -- however, as mentioned in Section \ref{sec:intro}
a \textsl{second level} approach produces 
much more accurate results (roughly speaking, accuracy is related to the ability,
given a non-random PRNG, of recognizing its sequences as non-random, 
see details in \cite{PareschiRS07}).
%\smallskip\par 

It is worth noting  that the following approach can be
applied when $d^{asin}_{tv}$ or $p_{\chi^2}$ are 
\textsl{slightly} outside acceptance region (\eg $p_{\chi^2}\in(10^{-4}, 
10^{-2}$), 
what suggests rejecting $\mathcal{H}_0$ but is not a \textsl{strong evidence}):
double the length of the sequence, take new output from the PRNG and apply the test again.
Repeat (at most predefined number of times) the procedure until the evidence is strong (\eg $p_{\chi^2}<10^{-4}$)
or $\mathcal{H}_0$ is accepted (\eg $p_{\chi^2}>0.01$). This approach 
(called \textsl{``automation of statistical tests on randomness''}) was proposed 
and analyzed in \cite{Haramoto2009}.
 


% 
% 
%  We indicate thresholds f 
%  
%  
% Values larger then pre-specified level of significans
%  
%  Instead of fixing the threshold for $d^{tv}, d^{sep}$ and $T^{asin}$, we 
% simply calculate these measures/statistics and compare several PRNGs relatively.





% 
% Powyższą wartość możemy wyliczyć ze wzoru (\ref{eq:prob_sasin}).
% 
% Druga miara, $\nu^{asin}_n$,  reprezentuje rozkład empiryczny, wyznaczony w testach. Określamy

==> sections/arcsine_tester_old_LIL.tex <==
In this Section we will show how to exploit the theoretical properties of random walks discussed in preceding sections
to design a practical routine for testing PRNGs. We briefly describe the approach based on Arcsine Law we employ
in experiments presented in Section \ref{sec:experiments}. For the sake of completeness we will also recall some basic
facts about the method of evaluating PRNGs presented in \cite{Wang2015}. Finally, we will perform the analysis
of approximation errors that occur in our testing procedure.

\subsection{Arcsine Law based testing}
\label{subsec:arcsineTests}

 
\pl{tutaj nie daje wszystkiego na czerwono, ale duzo zmienilem tutaj 22.10.2018}

The general idea of tests is clear: take a sequence of bits generated by PRNG (treat them as $-1$ and $+1$)
and compare empirical distributions with distributions for truly random numbers (which are known).
Given the null hypothesis $\mathcal{H}_0$ that the sequence was randomly generatated
(vs. $\mathcal{H}_A$: that the sequence was not randomly 
generated) 
%the Arcsine Law  (Theorem \ref{twr:arcsine}) implies that 
the distribution of 
% PRNG produced really
% 
% we will compare it to Arcsine Law given in Theorem \ref{twr:arcsine}. 
%For given $X_1,\ldots, X_n$ let
%\begin{equation}
%D_k = \mathbbm{1}\left(S_k > 0 \vee S_{k-1}>0 \right), k=1,2,\ldots,n.
%\end{equation}
%$D_k$ is equal to 1 if in $k$-th step number of ones prevails number of zeros
%(\textcolor{red}{traktując remisy tak jak w paragrafie \ref{sec:asin}}) and 0 otherwise.
%Let us define 
\begin{equation*}
 \Sasin{n} = \frac{1}{n} \sum_{k=1}^n D_k \in[0,1].
\end{equation*}
(a fraction of time instants at which ones prevail zeros) follows the Arcsine Law (Theorem \ref{twr:arcsine}),
\ie we can conclude that  \textsl{for large } $n$ we have 
\begin{equation}\label{eq:prob_sasin}
%\begin{split}
% \label{eq:prob_sasin}
%  \Pro{\Sasin{n} \in (a,b)} &\approx \frac{1}{\pi} \int_a^b \frac{dt}{\sqrt{t(1-t)}}\\
%  &= \frac{2}{\pi}\arcsin(\sqrt{b}) - \frac{2}{\pi}\arcsin(\sqrt{a}).
%\end{split}
\Pro{\Sasin{n} \in (a,b)} \approx \frac{1}{\pi} \int_a^b \frac{dt}{\sqrt{t(1-t)}} = \frac{2}{\pi}\arcsin(\sqrt{b}) - \frac{2}{\pi}\arcsin(\sqrt{a}).
\end{equation}
(we will be more specific on ``$\approx$'' in Section \ref{sec:err_analysis}).
We follow \textsl{second-level} testing approach \cite{PareschiRS07}, \cite{Pareschi2007}, \ie we take into account several results from the same test over 
different sequences. To test PRNG we generate $m$ sequences of length $n$ each. We obtain thus $m$ realizations of a variable $\Sasin{n}$, the $j$-th 
replication is denoted by $\Sasin{{n,j}}$. We fix some partition of  [0,1]
and count the number of realizations of $\Sasin{n}$ which 
are in a given interval. In our tests we will use  $(s+1)$ 
element partition $\mathcal{P}^{asin}_s = \{ P^{asin}_1,   \ldots, P^{asin}_{s+1}\}$, 
where
\begin{equation*}
\begin{split}
  P^{asin}_1 &= \left[0, \frac{1}{2s}\right),\\
  P^{asin}_i &= \left[\frac{2i-3}{2s}, \frac{2i-1}{2s} \right),\ \ \ 2 \leq i \leq s,\\
  P^{asin}_{s+1} &= \left[1- \frac{1}{2s},1\right].
\end{split}
\end{equation*}
Now we define  measures $\mu^{asin}_n , \nu^{asin}_n $,
 $E_i$ 
 (expected number of observations within $P^{asin}_i$) and 
 $O_i$ (the number of observations within $P^{asin}_i$):
 for $0 \leq i \leq s+1$,
\begin{align}
\mu^{asin}_n \left( P^{asin}_i \right) & =  \Pro{\Sasin{n} \in P^{asin}_i}, \quad E_i=m \cdot \mu_n^{asin}(P_i^{asin}),
\label{eq:mu_asin} \\ 
\nu^{asin}_n \left( P^{asin}_i \right) &= \frac{|\{ j:\ \Sasin{{n,j}} \in  P^{asin}_i, 1 \leq j \leq m\}|}{m},
 \quad O_i=m \cdot \nu_n^{asin}(P_i^{asin}). \label{eq:emp_asin}
\end{align}
We perform Pearson's goodness-of-fit test, which uses the following 
test statistic:
\begin{equation}
\label{eq:chi_asin2}
 T^{asin} = \sum_{i=1}^{s+1} \frac{(O_i - E_i)^2}{E_i}
 = m \cdot\sum_{A\in \mathcal{P}^{asin}_s} {(\mu_n(A) -\nu_n(A))^2\over 
 \mu_n(A)}.
\end{equation}
Under the null hypothesis, $T^{asin}$ 
has approximately $\chi^2(s)$ distribution.  
We calculate the correpsonding $p$-value 
$$p_{\chi^2} = \Pro{X>T^{asin}},$$
where $X$ has $\chi^2(s)$ distribution. 
Large values of $T^{asin}$ and small values of $p_{\chi^2}$ mean that PRNG is not good. 
Typically, we reject $\mathcal{H}_0$ (\ie we consider the 
test \textsl{failed}) if $p_{\chi^s}<\alpha,$ 
where $\alpha$ is a prescribed \textsl{level of significance}.
Note that the probability of rejecting 
$\mathcal{H}_0$  when the sequence is generated by a perfect random 
generator (so called \textsl{Type I error}) is $\alpha$.


\par 
Another approach is based on a \textsl{statistical distance 
based testing}, the approach was presented in \cite{Wang2015}.
We consider the statistic 
\begin{equation}
\label{eq:dtv}
 d_{tv}^{asin} =  {1\over 2} \sum_{A\in \mathcal{P}^{asin}_s} 
 |\mu_n(A) -\nu_n(A)|\in[0,1],
\end{equation}
 


\ie a total variation distance between the theoretical 
distribution $\mu^{asin}_n$ and the empirical 
distribution $\nu^{asin}_n $. Similarly, large values of 
$d_{tv}^{asin}$ indicate that PRNG is not good. 
Concerning \textsl{Type I error} we will make use 
of the following lemma (see Lemma 3 in \cite{devroye1983}
or its reformulation, Lemma 1 in \cite{Berend2012})
\begin{lem}\label{lem:devroy}
 Assume $\mathcal{H}_0$ and consider partition $\mathcal{P}_s^{asin}$, then  for all $\varepsilon \geq \sqrt{20 (s+1)/m} $ we have 
 $$\Pro{2d_{tv}^{asin} > \varepsilon} \leq 3 exp\left( -{m\varepsilon^2\over 25}\right).$$
\end{lem}



\medskip\par 
% 
% \pl{ASDF}
% and 
% 
% 
% % 
% % \begin{equation}
% % \label{eq:mu_asin}
% %  \mu^{asin}_n \left( P^{asin}_i \right) = P{\Sasin{n} \in P^{asin}_i}, 
% % \end{equation}
% % \begin{equation}
% %  \label{eq:emp_asin}
% %  \nu^{asin}_n \left( P^{asin}_i \right) = \frac{|\{ j:\ \Sasin{{n,j}} \in  P^{asin}_i, 1 \leq j \leq m\}|}{m}.
% % \end{equation}
% \noindent
% Measure $\mu^{asin}_n$ corresponds to the theoretical distribution and can 
% be approximately
% calculated by (\ref{eq:prob_sasin}), whereas 
% $\nu^{asin}_n$ represents empirical distribution obtained from tests.
% We will measure the distance  between these measures either using \textsl{total variation} or \textsl{separation} distance
%  defined for partition $\mathcal{P}$ as follows:
% %  
% % 
% % \textcolor{red}{ZMIENIC: If the PRNG is ``good'' then the measures should be close one to each other, what we will measure in various of ways.}
% % 
% % First, we will calculate \textsl{total variation} and \textsl{separation} distances defined for partition $\mathcal{P}$ as follows:
% \begin{align}
%  \label{eq:dtv_old}
%  d^{tv}_\mathcal{P}(\mu, \nu) &= \frac{1}{2} \sum_{A \in \mathcal{P}} |\mu(A) - \nu(A)|
%     %= \sum_{\substack{A \in \mathcal{P},\\ \mu(A) >\nu(A)}} \Big(\mu(A) - \nu(A)\Big),
%     ,\\
%  \label{eq:sep} 
% d^{sep}_\mathcal{P}(\mu, \nu) &= \max_{A \in \mathcal{P}}\left(1 - \frac{\mu(A)}{\nu(A)}\right).
% \end{align}
% Another approach is based on hypothesis testing. Using statistical terminology $\Sasin{{n,j}}$ will be called observations.
% Null hypothesis is that observations have distribution $\mu^{asin}_n$ , \ie that PRNG produces random bits.
% Define
% \begin{equation*}
%  O_i = |\{ j:\ \Sasin{{n,j}} \in  P^{asin}_i, 1 \leq j \leq m\}|,\ \ \ 0 \leq i \leq s+1,
% \end{equation*}
% the number of observations within $P^{asin}_i$ interval. Let $E_i$ denote expected number of observations within this interval,
% \ie $E_i=m\cdot\Pro{\Sasin{n}\in P^{asin}_i}$ (what is calculated from (\ref{eq:prob_sasin})). Assuming null hypothesis
% the statistic
% 

Summarizing, for given PRNG we generate $m$ sequences of length $n$ each. 
Then we choose $s$ (and thus a partition $\mathcal{P}^{asin}_s$),
calculate $d^{asin}_{tv}$
 and $T^{asin}$ together with its $p_{\chi^2}$-value. 
We specify thresholds for $p_{\chi^2}$-value   and 
$d^{tv}_\mathcal{P}$ indicating if the test \textsl{failed} or not 
(details in Section \ref{sec:experiments}).


\pl{TO DO: uwaga, ze to co robimy to dokladnie to samo co
w second-level testing, tzn., najpierw p-wartosci, a potem 
test jednostajnosci}


It is worth noting  that the following approach can be
applied when $d^{asin}_{tv}$ or $p_{\chi^2}$ are 
\textsl{slightly} outside acceptence region (\eg $p_{\chi^2}\in(10^{-4}, 10^{-2}$, 
what suggests rejecting $\mathcal{H}_0$ but is not a \textsl{strong evidence}):
double the length of the sequence, take new output from PRNG and apply the test again.
Repeat (at most predefined number of times) the procedure until the evidence is strong (\eg $p_{\chi^2}<10^{-4}$)
or $\mathcal{H}_0$ is accepted (\eg $p_{\chi^2}>0.01$). This approach 
(called \textsl{``automation of statistical tests on randomness''}) was proposed 
and analyzed in \cite{Haramoto2009}.
 


% 
% 
%  We indicate thresholds f 
%  
%  
% Values larger then pre-specified level of significans
%  
%  Instead of fixing the threshold for $d^{tv}, d^{sep}$ and $T^{asin}$, we 
% simply calculate these measures/statistics and compare several PRNGs relatively.







==> sections/experiments_all.tex <==




Total running times needed for generating and calculating statistics are given in tables.
Each simulation   was performed on one thread on 
twin Intel Xeon E5-2630 v2 CPUs (12 physical cores @2.60GHz) with 64 GB RAM.
Note that instead of simulating 10000 paths on one thread, it is possible 
to simulate \eg 1000 paths on 10 threads and then combine the results.
It would significantly decrease the total running times.
The source code of our implementation is available at \url{https://github.com/lorek/PRNG_Arcsine_test}.

In the following sections we provide the outcomes of performed tests 
as well as discussion and analysis of the  results.
The outcomes of experiments for each PRNG are summarized in tables in the following way.
The first row denotes the length $n$ of generated subsequences. For a subsequence of length $n_k$
the theoretical probability measure $\mu_{n_k}$ was calculated according to formula \eqref{eq:mu_asin}
or \eqref{eq:mu_lil} and the empirical measure $\nu_{n_k}$ according to (\ref{eq:emp_asin}) or \eqref{eq:emp_lil}
depending on considered characteristic. 
Successive columns contain the values of $d^{tv}(\mu_{n_k}, \nu_{n_k})$, $d^{sep}(\mu_{n_k}, \nu_{n_k})$,
$d^{sep}(\nu_{n_k}, \mu_{n_k})$ and $p$-value of the statistic (\ref{eq:chi_asin2}).
We provide both, $d^{sep}(\mu_{n_k}, \nu_{n_k})$ and $d^{sep}(\nu_{n_k}, \mu_{n_k})$, since -- despite phrase ``distance'' in its name -- 
separation distance $d^{sep}(\cdot, \cdot)$ is not symmetric.


\par 

 

% 
% on our flawed generator (including $J$ 
% statistic from \texttt{swalk}).
% The results were similar to ours - in all the cases (different sequences' 
% length) the corresponding $p$-value for statistic $J$ was 0.0 . The size of 
% the partion was automatically set to 998 (whereas we used $s=40$). 
% We also performed tests from NIST Test Suite - the flawed generator passed many of them, details given in next section.+


 

 
 

\subsection{BSD libc rand()}
Function \texttt{rand} from BSD system standard library has used originally $LCG(2^{31}, 1103515245, 12345)$ 
and  it does not truncate its output, \ie it returns all bits of generated numbers. 
Hence, in our experiments with BSD \texttt{rand} we also adopt the full output produced by this LCG. 
Tables \ref{tab:bsd_asin} and \ref{tab:bsd_lil} clearly depict why the original implementation of this generator
has been changed.% quickly.
 


% 
% \begin{table*}[t!]
% \centering
%  \caption{Results of ASIN test for initial version of PRNG from BSD libc. \texttt{ Time: 316.2 hrs}}
%  \label{tab:bsd_asin}
% \begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|}   
%  \hline 
%  
%       %n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{25}$ &  $2^{26}$\\ \hline
%       n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
%       tv &  0.2613 & 0.2805 & 0.3078 & 0.3332 & 0.3331 & 0.4073 & 0.4466 & 0.497 & 0.5584\\ \hline
%    sep1 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 \\ \hline
%    sep2 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
%   p-val &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline
% \end{tabular}  
% \end{table*}
% 
% 
% \begin{table*}[t!]
% \centering
%  \caption{Results of LIL test for initial version of PRNG from BSD libc. \texttt{ Time: 297.20 hrs}}
%  \label{tab:bsd_lil}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}  
%  \hline 
%      n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
%     tv & 0.0411 & 0.0403 & 0.0425 & 0.0453 & 0.04 & 0.0568 & 0.0605 & 0.0905 & 0.1053 \\ \hline
%    sep1 &  0.1868 & 0.1924 & 0.2373 & 0.2499 & 0.2163 & 0.3551 & 0.2752 & 0.3989 & 0.5135\\ \hline
%    sep2 &  0.1897 & 0.1827 & 0.1711 & 0.1644 & 0.1843 & 0.2420 & 0.2664 & 0.3253 & 0.3273\\ \hline
%   p-val &  0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\ \hline
% \end{tabular}  
% \end{table*}



\begin{table*}[t!]
\centering
 \caption{Results of ASIN test for initial version of PRNG from BSD libc. \texttt{ Time: 69m 10s} }
 \label{tab:bsd_asin}
\begin{tabular} {|c|c|c|c|c|c|c|}   
 \hline 
      n &  $2^{21}$ &  $2^{22}$ &  $2^{23}$ &  $2^{24}$ &  $2^{25}$ &  $2^{26}$\\ \hline
     tv &  0.0424 & 0.0499 & 0.0495 & 0.0464 & 0.0448 & 0.0411\\ \hline
   sep1 &  0.1798 & 0.2036 & 0.2303 & 0.2065 & 0.2093 & 0.1868\\ \hline
   sep2 &  0.1919 & 0.2276 & 0.1729 & 0.1793 & 0.2172 & 0.1897\\ \hline
  p-val &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline
\end{tabular}  
\end{table*}

\begin{table*}[t!]
\centering
 \caption{Results of LIL test for initial version of PRNG from BSD libc. \texttt{ Time: 65m 40s}}
 \label{tab:bsd_lil}
\begin{tabular} {|c|c|c|c|c|c|c|}   
 \hline 
      n &  $2^{21}$ &  $2^{22}$ &  $2^{23}$ &  $2^{24}$ &  $2^{25}$ &  $2^{26}$\\ \hline
     tv &  0.1828 & 0.2152 & 0.2381 & 0.2437 & 0.2565 & 0.2613\\ \hline
   sep1 &  0.9903 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
   sep2 &  0.3629 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
  p-val &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline
\end{tabular}  
\end{table*}

% 
% \begin{table*}[t!]
% \centering
%  \caption{Results of ASIN test for initial version of PRNG from BSD libc.}
%  \label{tab:bsd_asin_old}
% \begin{tabular} {|c|c|c|c|c|c|c|}   
%  \hline 
% \rowcolor{lightgray}      n &  $2^{21}$ &  $2^{22}$ &  $2^{23}$ &  $2^{24}$ &  $2^{25}$ &  $2^{26}$\\ \hline
% \rowcolor{lightgray}     tv &  0.0883 &  0.0980 &  0.0862 &  0.0951 &  0.0936 &  0.1081\\ \hline
% \rowcolor{lightgray}   sep1 &  0.3402 &  0.3979 &  0.4111 &  0.4980 &  0.4346 &  0.4751\\ \hline
% \rowcolor{lightgray}   sep2 &  0.3634 &  0.4198 &  0.3053 &  0.2805 &  0.3424 &  0.4070\\ \hline
% \rowcolor{lightgray}  p-val &  0.1829 &  0.0326 &  0.1874 &  0.1767 &  0.1181 &  0.0051\\ \hline
% \end{tabular}  
% \end{table*}
% 
% \begin{table*}[t!]
% \centering
%  \caption{Results of LIL test for initial version of PRNG from BSD libc.}
%  \label{tab:bsd_lil_old}
% \begin{tabular} {|c|c|c|c|c|c|c|}   
%  \hline 
% \rowcolor{lightgray}      n &  $2^{21}$ &  $2^{22}$ &  $2^{23}$ &  $2^{24}$ &  $2^{25}$ &  $2^{26}$\\ \hline
% \rowcolor{lightgray}     tv &  0.1956 &  0.2191 &  0.2472 &  0.2539 &  0.2464 &  0.2707\\ \hline
% \rowcolor{lightgray}   sep1 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
% \rowcolor{lightgray}   sep2 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
% \rowcolor{lightgray}  p-val &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline
% \end{tabular}  
% \end{table*}




From the obtained results one can easily notice that even for short sequences the output of BSD \texttt{rand} function
turns out to be far from truly random. Also all the statistics of \texttt{swalk\_RandomWalk1} from \texttt{TestU01} 
conducted for sequences of length $2^{26}$ indicate that this is not a good PRNG (see Table \ref{tab:tesu01_all}).
The reason behind that is the LCG uses modulus $2^{31}$, 
what implies that the period of $d$ least significant bits equals to $2^d$. As a result the number of 0s and 1s
is fairly close to each other what is easily recognized by the tests based on properties of random walks.
It is worth
mentioning that this flaw is slightly more evident in the outcomes of tests based on $\Slil{n}$ characteristic, 
which outperforms those based on $\Sasin{n}$ in this case. 

Similarly, the results (not included here) for RANDU (which is defined as $MCG(2^{31},65539)$) are comparable to those for 
\texttt{rand} from BSD system standard library.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Microsoft Visual C++ rand() %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Microsoft Visual C++ rand()}
\label{subsec:expMSVisual}
Function \texttt{rand} in Microsoft Visual C++ is based on $LCG(2^{32}, 214013, 2531011)$  linear congruential generator). It differs from
an ordinary LCG in that it returns only the most significant 15 bits.
This PRNG is one of those tested in \cite{Wang2015}. As the authors in \cite{Wang2015},
we discard the least significant 7 bits of numbers
produced by the \texttt{rand} function (\ie we take into account only the MSB on positions  
from 23 to 30  of the
number generated by LCG). The results of performed tests are presented in Tables \ref{tab:svis_asin} and \ref{tab:svis_lil}.

\begin{table*}[t!]
\centering
 \caption{Results of ASIN  test for PRNG in MS Visual C++. \texttt{Time: 377 hrs}}
 \label{tab:svis_asin}
\begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
 \hline
     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
     tv &  0.0289 &  0.0387 &  0.0615 &  0.0768 &  0.0848 &  0.0928 &  0.0965 &  0.1870 &  0.2093\\ \hline
   sep1 &  0.2030 &  0.1548 &  0.1952 &  0.2605 &  0.3664 &  0.4210 &  0.5528 &  0.6533 &  0.8163\\ \hline
   sep2 &  0.1780 &  0.2260 &  0.2524 &  0.2364 &  0.2841 &  0.3160 &  0.4336 &  0.6112 &  0.4328\\ \hline
  p-val &  0.0148 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline 
\end{tabular}  
\end{table*}

\begin{table*}[t!]
\centering
 \caption{Results of LIL test for PRNG in MS Visual C++. \texttt{Time: 397 hrs}}
 \label{tab:svis_lil}
\begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
 \hline 
     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
     tv &  0.0348 & 0.0510 & 0.0938 & 0.1234 & 0.1672 & 0.2423 & 0.3100 & 0.4991 & 0.9500\\ \hline
   sep1 &  0.2831 & 0.7419 & 0.9731 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000\\ \hline
   sep2 &  0.2670 & 0.1400 & 0.2635 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000\\ \hline
  p-val &  0.0001 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000\\ \hline
\end{tabular}  
\end{table*}



% 
% \begin{table*}[t!]
% \centering
%  \caption{Results of ASIN  test for PRNG in MS Visual C++.}
%  \label{tab:svis_asin_old}
% \begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
%  \hline
%      n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
%      tv &  0.0289 &  0.0387 &  0.0615 &  0.0768 &  0.0848 &  0.0928 &  0.0965 &  0.1870 &  0.2093\\ \hline
%    sep1 &  0.2030 &  0.1548 &  0.1952 &  0.2605 &  0.3664 &  0.4210 &  0.5528 &  0.6533 &  0.8163\\ \hline
%    sep2 &  0.1780 &  0.2260 &  0.2524 &  0.2364 &  0.2841 &  0.3160 &  0.4336 &  0.6112 &  0.4328\\ \hline
%   p-val &  0.0128 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline 
% \end{tabular}  
% \end{table*}
% 
% \begin{table*}[t!]
% \centering
%  \caption{Results of LIL test for PRNG in MS Visual C++.}
%  \label{tab:svis_lil_old}
% \begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
%  \hline 
%      n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
%      tv &  0.0350 &  0.0512 &  0.0938 &  0.1234 &  0.1672 &  0.2423 &  0.3100 &  0.4991 &  0.9500\\ \hline
%    sep1 &  0.2831 &  0.7419 &  0.9731 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
%    sep2 &  0.2670 &  0.1416 &  0.2635 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
%   p-val &  0.0001 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline
% \end{tabular}  
% \end{table*}
% 


Notice that this LCG has period $2^{31}$ and from single call of \texttt{rand} we get $8 = 2^3$ bits. 
This implies that when generating a sequence of bits of length $2^{34}$ we go through the full cycle of generator.
Hence, each combination of 8 bits has to be generated the same number of times, what leads to the conclusion that
after $2^{34}$ steps the random walk always returned to 0. This is evident in test results for characteristic $\Slil{n}$.
For $n=2^{34}$ all observations fall into the interval $[0, 0.05)$, for which the theoretical measure
$\mu^{lil}_n([0, 0.05)) \sim 0.05$, thus $d^{tv}(\mu^{lil}_n, \nu^{lil}_n) \approx 0.95$.

It is clear that generators with short periods cannot be used for generating large amounts of pseudorandom numbers.
However, observe that the PRNG analyzed in this section  fails the tests even for $n=2^{26}$ and generating
a random walk of this length requires only $2^{23} / 2^{31} = 1/2^8 \approx 0.4\%$ of the full period 
Thus, this PRNG cannot be considered as random even when restricting only to generators with short periods.
What is \textbf{surprising}, this PRNG passes the NIST Test Suite \cite{NISTtests}, as pointed out in \cite{Wang2015}.
Note  that for  $n=2^{26}$ none of the  $p$-values of \texttt{swalk\_RandomWalk1} from \texttt{TestU01} suggests rejecting the hypothesis that 
it is a good PRNG).

We also conducted (not included here) the experiments 
for  the procedure \texttt{rand} from standard library in Borland C/C++ (which implements $LCG(2^{32},22695477, 1)$).
The outcomes are very akin to those for standard PRNG in MS Visual C++.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% GLIBC rand() %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{GLIBC standard library rand()}
Function \texttt{rand} in GNU C Library makes use of more complicated generator than these described in the preceding
sections. Its state is determined by 34 numbers $x_i, x_{i+1},\ldots, x_{i+33}$. The PRNG is seeded with some random
number $s$, $0 \leq s \leq 2^{31}$, and its initial state is given by
\begin{align*}
  x_0 & = s && \\
  x_i & = 16807 x_{i-1} \mod (2^{31}-1), && 0 < i < 31\\
  x_i & = x_{i-31}, && i \in \{31,32,33\}.
\end{align*}
The successive values $x_i$ are calculated according to the formula 
\[ x_i = (x_{i-3} + x_{i-31}) \mod2^{32}. \]
$k$-th call to the function \texttt{rand} results in returning $x_{k+343} \gg 1$ (where $\gg$ is a right logical shift operator).
%, where $x >> k$ denotes shifting the binary representation of x to the right by k bits 
%\marginpar{\tiny\textcolor{red}{gdzies wprowadzic oznaczenia $\gg$}}


\begin{table*}[t!]
\centering
 \caption{Results of ASIN test for GNU C standard library generator. \texttt{ Time: 313.2 hrs}}
 \label{tab:mojkomp_asin}
\begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
 \hline
     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
     tv &  0.0238 & 0.0266 & 0.0286 & 0.0247 & 0.0178 & 0.0279 & 0.0232 & 0.0257 & 0.0255\\ \hline
   sep1 &  0.2079 & 0.1187 & 0.1666 & 0.1186 & 0.1481 & 0.1780 & 0.1879 & 0.1514 & 0.1405\\ \hline
   sep2 &  0.1491 & 0.1566 & 0.1785 & 0.1606 & 0.1063 & 0.1482 & 0.1744 & 0.1421 & 0.1961\\ \hline
  p-val &  0.4731 & 0.2100 & 0.1758 & 0.3663 & 0.9744 & 0.1206 & 0.4593 & 0.1563 & 0.2389\\ \hline 
\end{tabular}  
\end{table*}

\begin{table*}[t!]
\centering
 \caption{Results of LIL test for GNU C standard library generator. \texttt{ Time: 295.4 hrs}}
 \label{tab:mojkomp_lil}
\begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
 \hline 
     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
     tv &  0.0215 & 0.0272 & 0.0226 & 0.023 & 0.021 & 0.0212 & 0.0325 & 0.0235 & 0.0220\\ \hline
   sep1 &  0.3828 & 0.1802 & 0.2838 & 0.1978 & 0.1508 & 0.1853 & 0.3451 & 0.3737 & 0.2696\\ \hline
   sep2 &  0.1449 & 0.2568 & 0.2735 & 0.1970 & 0.1831 & 0.2521 & 0.3456 & 0.2284 & 0.1327\\ \hline
  p-val &  0.6052 & 0.0714 & 0.5685 & 0.5729 & 0.7853 & 0.5988 & 0.0019 & 0.4231 & 0.7914\\ \hline
\end{tabular}  
\end{table*}

% 
% \begin{table*}[t!]
% \centering
%  \caption{Results of ASIN test for GNU C standard library generator.}
%  \label{tab:mojkomp_asin_old}
% \begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
%  \hline
% \rowcolor{lightgray}     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
% \rowcolor{lightgray}     tv &  0.0287 &  0.0217 &  0.0264 &  0.0228 &  0.0202 &  0.0289 &  0.0237 &  0.0254 &  0.0230\\ \hline
% \rowcolor{lightgray}   sep1 &  0.1157 &  0.1249 &  0.1629 &  0.1186 &  0.1661 &  0.1717 &  0.1306 &  0.1316 &  0.1405\\ \hline
% \rowcolor{lightgray}   sep2 &  0.1754 &  0.1909 &  0.1436 &  0.1869 &  0.1110 &  0.1344 &  0.1786 &  0.1262 &  0.1879\\ \hline
% \rowcolor{lightgray}  p-val &  0.0649 &  0.5511 &  0.2565 &  0.4887 &  0.7967 &  0.1115 &  0.5880 &  0.2599 &  0.3930\\ \hline 
% \end{tabular}  
% \end{table*}
% 
% \begin{table*}[t!]
% \centering
%  \caption{Results of LIL test for GNU C standard library generator.}
%  \label{tab:mojkomp_lil_old}
% \begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
%  \hline 
% \rowcolor{lightgray}     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
% \rowcolor{lightgray}     tv &  0.0185 &  0.0243 &  0.0242 &  0.0244 &  0.0210 &  0.0220 &  0.0330 &  0.0237 &  0.0221\\ \hline
% \rowcolor{lightgray}   sep1 &  0.2593 &  0.1640 &  0.1844 &  0.2573 &  0.2010 &  0.1853 &  0.2882 &  0.4129 &  0.2563\\ \hline
% \rowcolor{lightgray}   sep2 &  0.0807 &  0.2133 &  0.2299 &  0.2060 &  0.1839 &  0.2361 &  0.3456 &  0.2078 &  0.1405\\ \hline
% \rowcolor{lightgray}  p-val &  0.9627 &  0.4878 &  0.5225 &  0.3022 &  0.6978 &  0.5382 &  0.0009 &  0.4903 &  0.7901\\ \hline
% \end{tabular}  
% \end{table*}

For our tests we took all 31 bits outputted by PRNG. From the results gathered in Tables \ref{tab:mojkomp_asin}
and \ref{tab:mojkomp_lil} one may conclude that ASIN test gives no reason for rejecting the hypothesis that
the sequences generated by the analyzed PRNG are random. In the case of LIL test, the results for $n=2^{34}$ and $n=2^{33}$
may also suggest that this PRNG is good. However, for $n=2^{32}$ we can observe an evident deviation,
namely the $p$-value is very small, only about $1/1000$. This can be a matter of chance -- with probability $1/1000$ this
could happen even for a truly random generator. However, take a look on $p$-values for ten data subsets of size 1000
(\ie each sample consists of 1000 sequences). We have $0.9313$, $0.0949$, $0.8859$, $0.1739$, $0.3675$, $0.0334$, $0.0321$,
$0.1824$, $0.0017$, $0.6205$.  As we can see, 4 out of 10 $p$-values are below $0.1$. The probability that for truly random
sequences at least 4 $p$-values fall into that interval is
\[ 1 - \sum_{i=0}^3 \binom{10}{i} \left(\frac{1}{10}\right)^{i} \left(1 - \frac{1}{10}\right)^{10-i} \approx 0.0016~. \]
This suggests that the GLIBC standard library PRNG may contain some hidden flaws. 
Note that for $n=2^{36}$ no flaws were detected using   statistics of \texttt{swalk\_RandomWalk1} from \texttt{TestU01},
see Table \ref{tab:tesu01_all}.

However, despite the issue pointed above, the implementation of \texttt{rand} function considered in this section
appears to be the best among these already tested by us.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Minstd %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Minstd}
Minstd (abbr. from \textit{minimal standard generator}) is based on MCG with parameters recommended by Park and Miller
in \cite{Park1988}. The authors' goal was to develop a simple generator, not necessarily perfect, but fast, simple to
implement and suitable for most common applications. As a result they proposed $MCG(2^{31}-1, 16807)$.
%For generating binary sequences eight most significant bits returned by the PRNG were used.
%The results of experimental testing are shown in Tables \ref{tab:minstd_asin} and \ref{tab:minstd_lil}.
% 
% \begin{table*}[t!]
% \centering
%  \caption{Results of arcsine test for Minstd generator with multiplier 16807.}
%  \label{tab:minstd_asin}
% \begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
%  \hline
%      n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
%      tv &  0.0321 &  0.0321 &  0.0402 &  0.0725 &  0.0917 &  0.1116 &  0.1648 &  0.2003 &  0.2109\\ \hline
%    sep1 &  0.1172 &  0.1686 &  0.1407 &  0.2985 &  0.2880 &  0.6670 &  0.5203 &  0.7345 &  0.8486\\ \hline
%    sep2 &  0.1302 &  0.1490 &  0.2420 &  0.3986 &  0.4051 &  0.3735 &  0.3822 &  0.5352 &  0.3894\\ \hline
%   p-val &  0.0360 &  0.0203 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline
% \end{tabular}  
% \end{table*}
% 
% \begin{table*}[t!]
% \centering
%  \caption{Results of LIL test for Minstd generator with multiplier 16807.}
%  \label{tab:minstd_lil}
% \begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
%  \hline 
%      n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
%      tv &  0.0370 &  0.0622 &  0.0823 &  0.1120 &  0.1877 &  0.2002 &  0.3538 &  0.3194 &  0.9500\\ \hline
%    sep1 &  0.5035 &  0.5465 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
%    sep2 &  0.1444 &  0.2366 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
%   p-val &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline
% \end{tabular}  
% \end{table*}
In their later work from 1993, Park and Miller \cite{Park1993} suggested that it would be better to use 
the multiplier $48271$.
However, changing the multiplier does not affect our tests much. 
In Tables \ref{tab:nminstd_asin} and \ref{tab:nminstd_lil} the results for $48271$ are presented,
and those for $16807$ (not included here) are similar. 
 

\begin{table*}[t!]
\centering
 \caption{Results of ASIN test for Minstd generator with multiplier 48271. }
 %\textcolor{red}{NewMinstd3 sie robi! jak nie zdazy, damy $2^26$}
 \label{tab:nminstd_asin}
\begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
 \hline
     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
     tv &  0.0318 &  0.0430 &  0.0477 &  0.0982 &  0.1303 &  0.0918 &  0.0848 &  0.1131 &  0.2089\\ \hline
   sep1 &  0.1607 &  0.1467 &  0.1901 &  0.3803 &  0.4280 &  0.3845 &  0.4583 &  0.3975 &  0.8079\\ \hline
   sep2 &  0.1828 &  0.1719 &  0.2120 &  0.2548 &  0.3449 &  0.3179 &  0.3192 &  0.3186 &  0.4579\\ \hline
  p-val &  0.0115 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline
\end{tabular}  
\end{table*}

\begin{table*}[t!]
\centering
 \caption{Results of LIL test for Minstd generator with multiplier 48271.  }
 %\textcolor{red}{NewMinstd3 sie robi! jak nie zdazy, damy $2^26$}
 \label{tab:nminstd_lil}
\begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
 \hline 
     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
     tv &  0.0372 &  0.0563 &  0.0590 &  0.2573 &  0.2879 &  0.3408 &  0.3167 &  0.3434 &  0.9500\\ \hline
   sep1 &  0.3298 &  0.4839 &  0.9328 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
   sep2 &  0.3843 &  0.1850 &  0.2207 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
  p-val &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline
\end{tabular}  
\end{table*}
For the ASIN tests the total variation distance between theoretical and empirical measures decreased in most cases
after changing the multiplier, especially for longer sequences. But in the case of LIL tests the opposite change occurred. 
Thus, based on these results it is hard to say whether this modification brings significant improvement. Nevertheless,
$\chi^2$ test in both cases shows that Minstd is not a sound PRNG. 
This can also be seen in statistics of \texttt{swalk\_RandomWalk1} from 
\texttt{TestU01} conducted for sequences of length $2^{26}$, statistics H and C indicate that there can be some flaws in this 
PRNG, see Table \ref{tab:tesu01_all}.

Despite its weaknesses, Minstd became a part C++11 standard library. It is implemented by the classes
\texttt{std::minstd\_rand0} (with multiplier 16807) and \texttt{std::minstd\_rand} (with multiplier 48271).


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Mersene Twister %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Mersenne Twister}
Mersenne Twister generator was tested using the built-in implementation in C++11. 
We chose 64-bit version of the PRNG
\ie class \texttt{std::mt19937\_64}. 
%%%It is a minor modification of 32-bit variant characterized in Section \ref{subsec:prng},
%%% adapted to architectures with 8-byte words. 
In tests all 64 bits returned by a single call to the generator were used.
\begin{table*}[t!]
\centering
 \caption{Results of ASIN test for C++11 implementation of MT19937-64 generator. \texttt{ Time: 309.1 hrs}}
 \label{tab:twister_asin}
\begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
 \hline
  n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
  tv &  0.0272 & 0.0245 & 0.0226 & 0.0279 & 0.0273 & 0.0223 & 0.0273 & 0.0233 & 0.0252\\ \hline
  sep1 &  0.1421 & 0.1666 & 0.1167 & 0.1824 & 0.1938 & 0.1571 & 0.1760 & 0.1397 & 0.1573\\ \hline
  sep2 &  0.1133 & 0.1195 & 0.1056 & 0.1399 & 0.1209 & 0.1315 & 0.1391 & 0.1065 & 0.1444\\ \hline
  p-val &  0.2548 & 0.6674 & 0.8907 & 0.1014 & 0.1287 & 0.7727 & 0.1002 & 0.7447 & 0.2523\\ \hline
\end{tabular}  
\end{table*}

\begin{table*}[t!]
\centering
 \caption{Results of LIL test for C++11 implementation of MT19937-64 generator. \texttt{ Time: 291.5 hrs}}
 \label{tab:twister_lil}
\begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
 \hline 
     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
     tv &  0.0229 & 0.0243 & 0.0234 & 0.0207 & 0.0251 & 0.0297 & 0.0287 & 0.0309 & 0.0225\\ \hline
   sep1 &  0.1606 & 0.2400 & 0.1689 & 0.2890 & 0.1458 & 0.1853 & 0.2712 & 0.2318 & 0.1795\\ \hline
   sep2 &  0.2106 & 0.1458 & 0.2017 & 0.1228 & 0.1839 & 0.2492 & 0.1951 & 0.1748 & 0.1559\\ \hline
  p-val &  0.5440 & 0.6035 & 0.4630 & 0.8106 & 0.4609 & 0.0653 & 0.0593 & 0.0077 & 0.7745\\ \hline
\end{tabular}  
\end{table*}
% 
% \begin{table*}[t!]
% \centering
%  \caption{Results of ASIN test for C++11 implementation of MT19937-64 generator.}
%  \label{tab:twister_asin_old}
% \begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
%  \hline
% \rowcolor{lightgray}     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
% \rowcolor{lightgray}     tv &  0.0271 &  0.0245 &  0.0226 &  0.0281 &  0.0276 &  0.0228 &  0.0271 &  0.0230 &  0.0255\\ \hline
% \rowcolor{lightgray}   sep1 &  0.1421 &  0.1606 &  0.1167 &  0.1824 &  0.1938 &  0.1571 &  0.1760 &  0.1397 &  0.1573\\ \hline
% \rowcolor{lightgray}   sep2 &  0.1133 &  0.1195 &  0.1056 &  0.1399 &  0.1256 &  0.1287 &  0.1391 &  0.0994 &  0.1444\\ \hline
% \rowcolor{lightgray}  p-val &  0.2755 &  0.6823 &  0.8804 &  0.0801 &  0.1267 &  0.7343 &  0.1094 &  0.7596 &  0.2029\\ \hline
% \end{tabular}  
% \end{table*}
% \begin{table*}[t!]
% \centering
%  \caption{Results of LIL test for C++11 implementation of MT19937-64 generator.}
%  \label{tab:twister_lil_old}
% \begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
%  \hline 
% \rowcolor{lightgray}     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
% \rowcolor{lightgray}     tv &  0.0254 &  0.0264 &  0.0238 &  0.0234 &  0.0266 &  0.0265 &  0.0290 &  0.0299 &  0.0215\\ \hline
% \rowcolor{lightgray}   sep1 &  0.1853 &  0.2147 &  0.1689 &  0.3093 &  0.1887 &  0.2015 &  0.2877 &  0.2318 &  0.1953\\ \hline
% \rowcolor{lightgray}   sep2 &  0.2841 &  0.1696 &  0.1917 &  0.1282 &  0.2017 &  0.2492 &  0.1842 &  0.1541 &  0.1716\\ \hline
% \rowcolor{lightgray}  p-val &  0.2483 &  0.3690 &  0.5965 &  0.5066 &  0.2196 &  0.1495 &  0.0499 &  0.0189 &  0.8170\\ \hline
% \end{tabular}  
% \end{table*}
The results presented in Tables \ref{tab:twister_asin} and \ref{tab:twister_lil} give an explanation 
why the Mersenne Twister is one of the most popular PRNG used in practice. These outcomes 
give no arguments against the claim that the output of this PRNG is indeed truly random
(maybe only in case of $S^{LIL}$ there is some deviation from randomness in case $n=2^{33}$). 
This can also the case with in statistics of \texttt{swalk\_RandomWalk1} from 
\texttt{TestU01} conducted for sequences of length $2^{26}$,  see Table \ref{tab:tesu01_all}.
\medskip\par 
It is worth noting that the experiments for CMRG (not included here) gave similar results. 
Nevertheless, one should note that in \cite{Kim2008} 
the authors provide strong evidence that the output of CMRG is not sound.


%% TESTU1 Stats.  H, M, J , R, C

% \begin{table*}[t!]
% \centering \small
%  \caption{Results ($p$-values) of ASIN, LIL and \texttt{swalk\_RandomWalk1} statistics from \texttt{TestU01} for $n=2^{26}$.}
%  \label{tab:tesu01_all}
% \begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
%  \hline
%     PRNG\textbackslash Test &  ASIN 	&  LIL  	&  Statistic  H  	&  Statistic  M 		&  Statistic  J  	&  Statistic  R 	   &  Statistic  C  \\ \hline
%      BSD libc     &  0.0000 		&  0.0000 	& 0.000; 0.000 &  0.000; 0.000	 & 0.000; 0.000  & 0.000; 0.000  &	0.000; 0.000	  \\ 
% 		&    		&    			& 0.000; 0.000 &  0.000; 0.000	 & 0.000; 0.000  & 0.000; 0.000  &	0.000; 0.000	  \\ \hline
% 		
% 	
% MS Visual C++   &  0.0148 	& 0.0001 		& 0.920; 0.000 &  0.950; 0.000	 & 0.860; 0.000  & 0.230; 0.060  &	0.860; 0.020	  \\ 
% 		&  		&    			& 0.000; 0.002 &  0.000; 0.000	 & 0.000; 0.002  & 0.120; 0.530  &	0.020; 0.110	  \\ \hline
% 	
% 	
% 	
%       GNU C   &   0.4731		&  0.6052	& 0.080; 0.330 &  0.380; 0.170	 & 0.008; 0.008  & 0.660; 0.003  &	0.630; 0.007	  \\ 
% 		&  		&    			& 0.490; 0.740 &  0.320; 0.550	 & 0.008; 0.990  & 0.030; 0.010  &	0.110; 0.230	  \\ \hline
% 
% 		
%    Minstd 48271	  &  0.0115 		&  0.0000 		& 0.000; 0.310 &  0.013; 0.007	 & 0.290; 0.000  & 0.200; 0.270  &	0.490; 0.010	  \\ 
% 		&  	 		&    		& 0.000; 0.000 &  0.010; 0.994	 & 0.010; 0.530  & 0.280; 0.130  &	0.180; 0.080	  \\ \hline
% 		
%    MT19937-64 	  &  0.2548 	&  0.5540 		& 0.070; 0.007 &  0.580; 0.004	 & 0.340; 0.002   & 0.210; 0.270  &	0.150; 0.460	  \\ 
% 		&  		&    			& 0.030; 0.670 &  0.010; 0.080	 & 0.050; 0.029   & 0.760; 0.570  &	0.630; 0.270	  \\ \hline
% 
%   \textsl{Flawed}  &  0.0000	&  0.5558		& 0.540; 0.430 &  0.930; 0.370	 & 0.210; 0.910   & 0.270; 0.800  &	0.260; 0.550	  \\ 
% 		&  		&    			& 0.750; 0.310 &  0.570; 0.180	 & 0.330; 0.900   & 0.460; 0.750  &	0.470; 0.700	  \\ \hline
% 
% 		
% \end{tabular}  
% \end{table*}



==> sections/experiments_o.tex <==
% 4.1. BSD libc rand() -> "Rand"
% 4.2. Microsoft Visual C++ rand() -> "SVIS"
% 4.3. GLIBC stdlib rand() -> "C_PRG"
% 4.4. Minstd with multiplier 48271 -> "NewMinstd3"
% 4.5. Mersenne Twister - wbudowana implementacja C++11 -> "Mersenne"
% 4.6. Flawed -> "zepsuty"
% 
In this section we present and discuss a series of experimental results of testing some
widely used PRNGs implemented in standard libraries in various programming languages.
We performed both, ASIN and LIL  tests on generators including different implementations
of standard C/C++ linear congruential generators, the standard generator \textsc{rand} from
GNU C Library, Mersenne Twister, Minstd and CMRG generators.  
% Tables present results only for the generators which behave differently.
% \textcolor{red}{tutaj jakos opisac, ze niektorych nie ma w tabelkach bo maja ``same tendency''}
As our last example we propose some hypothetical weak PRNG which is clearly identified
by our ASIN test as non-random, whereas the LIL test fails to detect its obvious flaws. 

Each considered PRNG was tested by generating $m = 10000$ sequences of length $n = 2^{34}$
in most cases. The values of characteristics $\Sasin{r}$ or $\Slil{r}$
were calculated both for each sequence ($r=n$) as well as for subsequences of length $n/2, \ldots, n/2^{k}$
for some fixed value of $k$ depending on tested PRNG (usually $k = 8$). This approach,
called in \cite{Wang2015} \emph{snapshot testing} at points $2^{n}, \ldots, 2^{n/2^{k}}$, allows for
observing and comparing the values of analyzed parameters on different stages.
Finally, for each PRNG respective statistics and distances between theoretical and empirical distributions
were calculated, as described in detail in Sections \ref{subsec:arcsineTests} and \ref{subsec:lilTests}.
In our experimental analysis for tests based on characteristics $\Sasin{n}$ and $\Slil{n}$
we used partitions $\mathcal{P}^{asin}_{40}$ and $\mathcal{P}^{lil}_{40}$, respectively.

In the experiments we used our own implementations of tested PRNGs (except MT19937).
The generators were initialized with random seeds from \url{http://www.random.org} \cite{RandomOrg}
and each sequence was generated using different seed.
The source code of our implementation is available at \url{https://github.com/lorek/PRNG_Arcsine_test}.

In the following sections we provide the outcomes of performed tests 
as well as discussion and analysis of the  results.
The outcomes of experiments for each PRNG are summarized in tables in the following way.
The first row denotes the length $n$ of generated subsequences. For a subsequence of length $n_k$
the theoretical probability measure $\mu_{n_k}$ was calculated according to formula \eqref{eq:mu_asin}
or \eqref{eq:mu_lil} and the empirical measure $\nu_{n_k}$ according to (\ref{eq:emp_asin}) or \eqref{eq:emp_lil}
depending on considered characteristic. 
Successive columns contain the values of $d^{tv}(\mu_{n_k}, \nu_{n_k})$, $d^{sep}(\mu_{n_k}, \nu_{n_k})$,
$d^{sep}(\nu_{n_k}, \mu_{n_k})$ and $p$-value of the statistic (\ref{eq:chi_asin2}).
We provide both, $d^{sep}(\mu_{n_k}, \nu_{n_k})$ and $d^{sep}(\nu_{n_k}, \mu_{n_k})$, since -- despite phrase ``distance'' in its name -- 
separation distance $d^{sep}(\cdot, \cdot)$ is not symmetric.



\subsection{BSD libc rand()}
Function \texttt{rand} from BSD system standard library has used originally $LCG(2^{31}, 1103515245, 12345)$ 
and  it does not truncate its output, \ie it returns all bits of generated numbers. 
Hence, in our experiments with BSD \texttt{rand} we also adopt the full output produced by this LCG. 
Tables \ref{tab:bsd_asin} and \ref{tab:bsd_lil} clearly depict why the original implementation of this generator
has been changed.% quickly.
 



\definecolor{lightgray}{gray}{0.9}




  


\begin{table*}[t!]
\centering
<<<<<<< .mine
 \caption{Results of arcsine test for initial version of PRNG from BSD libc. \textsc{Time: 18975m35.059s}}
 \label{tab:bsd_asin}
\begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|}   
 \hline 
 
      %n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{25}$ &  $2^{26}$\\ \hline
      n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
      tv &  0.2613 & 0.2805 & 0.3078 & 0.3332 & 0.3331 & 0.4073 & 0.4466 & 0.497 & 0.5584\\ \hline
   sep1 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 \\ \hline
   sep2 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
  p-val &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline
  
\end{tabular}  

\end{table*}


\begin{table*}[t!]
\centering
 \caption{Results of LIL test for initial version of PRNG from BSD libc. \textsc{Time: 17836m37.911s}}
 \label{tab:bsd_lil}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}  
 \hline 
     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
    tv & 0.0411 & 0.0403 & 0.0425 & 0.0453 & 0.04 & 0.0568 & 0.0605 & 0.0905 & 0.1053 \\ \hline
   sep1 &  0.1868 & 0.1924 & 0.2373 & 0.2499 & 0.2163 & 0.3551 & 0.2752 & 0.3989 & 0.5135\\ \hline
   sep2 &  0.1897 & 0.1827 & 0.1711 & 0.1644 & 0.1843 & 0.2420 & 0.2664 & 0.3253 & 0.3273\\ \hline
  p-val &  0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\ \hline
\end{tabular}  
\end{table*}



\begin{table*}[t!]
\centering
 \caption{Results of arcsine test for initial version of PRNG from BSD libc.}
||||||| .r1435
 \caption{Results of arcsine test for initial version of PRNG from BSD libc.}
=======
 \caption{Results of ASIN test for initial version of PRNG from BSD libc.}
>>>>>>> .r1551
 \label{tab:bsd_asin_old}
\begin{tabular} {|c|c|c|c|c|c|c|}   
 \hline 
 
\rowcolor{lightgray}      n &  $2^{21}$ &  $2^{22}$ &  $2^{23}$ &  $2^{24}$ &  $2^{25}$ &  $2^{26}$\\ \hline
\rowcolor{lightgray}     tv &  0.0883 &  0.0980 &  0.0862 &  0.0951 &  0.0936 &  0.1081\\ \hline
\rowcolor{lightgray}   sep1 &  0.3402 &  0.3979 &  0.4111 &  0.4980 &  0.4346 &  0.4751\\ \hline
\rowcolor{lightgray}   sep2 &  0.3634 &  0.4198 &  0.3053 &  0.2805 &  0.3424 &  0.4070\\ \hline
\rowcolor{lightgray}  p-val &  0.1829 &  0.0326 &  0.1874 &  0.1767 &  0.1181 &  0.0051\\ \hline
\end{tabular}  

\end{table*}


\begin{table*}[t!]
\centering
 \caption{Results of LIL test for initial version of PRNG from BSD libc.}
 \label{tab:bsd_lil_old}
\begin{tabular} {|c|c|c|c|c|c|c|}   
 \hline 
\rowcolor{lightgray}      n &  $2^{21}$ &  $2^{22}$ &  $2^{23}$ &  $2^{24}$ &  $2^{25}$ &  $2^{26}$\\ \hline
\rowcolor{lightgray}     tv &  0.1956 &  0.2191 &  0.2472 &  0.2539 &  0.2464 &  0.2707\\ \hline
\rowcolor{lightgray}   sep1 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
\rowcolor{lightgray}   sep2 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
\rowcolor{lightgray}  p-val &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline
\end{tabular}  
\end{table*}

From the obtained results one can easily notice that even for short sequences the output of BSD \texttt{rand} function
turns out to be far from truly random. The reason behind that is the LCG uses modulus $2^{31}$, 
what implies that the period of $d$ least significant bits equals to $2^d$. As a result the number of 0s and 1s
is fairly close to each other what is easily recognized by the tests based on properties of random walks. It is worth
mentioning that this flaw is more evident in the outcomes of tests based on $\Slil{n}$ characteristic, which outperforms
those based on $\Sasin{n}$ in this case.

Similarly, the results (not included here) for RANDU (which is defined as $MCG(2^{31},65539)$) are comparable to those for 
\texttt{rand} from BSD system standard library.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Microsoft Visual C++ rand() %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Microsoft Visual C++ rand()}
\label{subsec:expMSVisual}
Function \texttt{rand} in Microsoft Visual C++ is based on $LCG(2^{32}, 214013, 2531011)$  linear congruential generator). It differs from
an ordinary LCG in that it returns only the bits on last 15 positions.
This PRNG is one of those tested in \cite{Wang2015}. As the authors in \cite{Wang2015},
we discard the least significant 7 bits of numbers
produced by the \texttt{rand} function (\ie we take into account only the MSB on positions 30..23 of the
number generated by LCG). The results of performed tests are presented in Tables \ref{tab:svis_asin} and \ref{tab:svis_lil}.

\begin{table*}[t!]
\centering
 \caption{Results of ASIN  test for PRNG in MS Visual C++.}
 \label{tab:svis_asin}
\begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
 \hline
     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
     tv &  0.0289 &  0.0387 &  0.0615 &  0.0768 &  0.0848 &  0.0928 &  0.0965 &  0.1870 &  0.2093\\ \hline
   sep1 &  0.2030 &  0.1548 &  0.1952 &  0.2605 &  0.3664 &  0.4210 &  0.5528 &  0.6533 &  0.8163\\ \hline
   sep2 &  0.1780 &  0.2260 &  0.2524 &  0.2364 &  0.2841 &  0.3160 &  0.4336 &  0.6112 &  0.4328\\ \hline
  p-val &  0.0128 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline 
\end{tabular}  
\end{table*}

\begin{table*}[t!]
\centering
 \caption{Results of LIL test for PRNG in MS Visual C++.}
 \label{tab:svis_lil}
\begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
 \hline 
     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
     tv &  0.0350 &  0.0512 &  0.0938 &  0.1234 &  0.1672 &  0.2423 &  0.3100 &  0.4991 &  0.9500\\ \hline
   sep1 &  0.2831 &  0.7419 &  0.9731 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
   sep2 &  0.2670 &  0.1416 &  0.2635 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
  p-val &  0.0001 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline
\end{tabular}  
\end{table*}

Notice that this LCG has period $2^{31}$ and from single call of \texttt{rand} we get $8 = 2^3$ bits. 
This implies that when generating a sequence of bits of length $2^{34}$ we go through the full cycle of generator.
Hence, each combination of 8 bits has to be generated the same number of times, what leads to the conclusion that
after $2^{34}$ steps the random walk always returned to 0. This is evident in test results for characteristic $\Slil{n}$.
For $n=2^{34}$ all observations fall into the interval $[0, 0.05)$, for which the theoretical measure
$\mu^{lil}_n([0, 0.05)) \sim 0.05$, thus $d^{tv}(\mu^{lil}_n, \nu^{lil}_n) \approx 0.95$.

It is clear that generators with short periods cannot be used for generating large amounts of pseudorandom numbers.
However, observe that the PRNG analyzed in this section  fails the tests even for $n=2^{26}$ and generating
a random walk of this length requires only $2^{23} / 2^{31} = 1/2^8 \approx 0.4\%$ of the full period. 
Thus, this PRNG cannot be considered as random even when restricting only to generators with short periods.
What is \textbf{surprising}, this PRNG passes the NIST Test Suite \cite{NISTtests}, as pointed out in \cite{Wang2015}.

We also conducted (not included here) the experiments 
for  the procedure \texttt{rand} from standard library in Borland C/C++ (which implements $LCG(2^{32},22695477, 1)$).
The outcomes are very akin to those for standard PRNG in MS Visual C++.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% GLIBC rand() %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{GLIBC standard library rand()}
Function \texttt{rand} in GNU C Library makes use of more complicated generator than these described in the preceding
sections. Its state is determined by 34 numbers $x_i, x_{i+1},\ldots, x_{i+33}$. The PRNG is seeded with some random
number $s$, $0 \leq s \leq 2^{31}$, and its initial state is given by
\begin{align*}
  x_0 & = s && \\
  x_i & = 16807 x_{i-1} \mod (2^{31}-1), && 0 < i < 31\\
  x_i & = x_{i-31}, && i \in \{31,32,33\}.
\end{align*}
The successive values $x_i$ are calculated according to the formula 
\[ x_i = (x_{i-3} + x_{i-31}) \mod2^{32}. \]
$k$-th call to the function \texttt{rand} results in returning $x_{k+343} \gg 1$ (where $\gg$ is a right logical shift operator).
%, where $x >> k$ denotes shifting the binary representation of x to the right by k bits 
%\marginpar{\tiny\textcolor{red}{gdzies wprowadzic oznaczenia $\gg$}}

\begin{table*}[t!]
\centering
<<<<<<< .mine
 \caption{Results of arcsine test for GNU C standard library generator. \textsc{Time: 18792m13.097s}}
||||||| .r1435
 \caption{Results of arcsine test for GNU C standard library generator.}
=======
 \caption{Results of ASIN test for GNU C standard library generator.}
>>>>>>> .r1551
 \label{tab:mojkomp_asin}
\begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
 \hline
     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
     tv &  0.0238 & 0.0266 & 0.0286 & 0.0247 & 0.0178 & 0.0279 & 0.0232 & 0.0257 & 0.0255\\ \hline
   sep1 &  0.2079 & 0.1187 & 0.1666 & 0.1186 & 0.1481 & 0.1780 & 0.1879 & 0.1514 & 0.1405\\ \hline
   sep2 &  0.1491 & 0.1566 & 0.1785 & 0.1606 & 0.1063 & 0.1482 & 0.1744 & 0.1421 & 0.1961\\ \hline
  p-val &  0.4731 & 0.2100 & 0.1758 & 0.3663 & 0.9744 & 0.1206 & 0.4593 & 0.1563 & 0.2389\\ \hline 
\end{tabular}  
\end{table*}

\begin{table*}[t!]
\centering
 \caption{Results of LIL test for GNU C standard library generator. \textsc{Time: 17724m21.168s}}
 \label{tab:mojkomp_lil}
\begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
 \hline 
     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
     tv &  0.0215 & 0.0272 & 0.0226 & 0.023 & 0.021 & 0.0212 & 0.0325 & 0.0235 & 0.0220\\ \hline
   sep1 &  0.3828 & 0.1802 & 0.2838 & 0.1978 & 0.1508 & 0.1853 & 0.3451 & 0.3737 & 0.2696\\ \hline
   sep2 &  0.1449 & 0.2568 & 0.2735 & 0.1970 & 0.1831 & 0.2521 & 0.3456 & 0.2284 & 0.1327\\ \hline
  p-val &  0.6052 & 0.0714 & 0.5685 & 0.5729 & 0.7853 & 0.5988 & 0.0019 & 0.4231 & 0.7914\\ \hline
\end{tabular}  
\end{table*}



\begin{table*}[t!]
\centering
 \caption{Results of arcsine test for GNU C standard library generator.}
 \label{tab:mojkomp_asin_old}
\begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
 \hline
\rowcolor{lightgray}     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
\rowcolor{lightgray}     tv &  0.0287 &  0.0217 &  0.0264 &  0.0228 &  0.0202 &  0.0289 &  0.0237 &  0.0254 &  0.0230\\ \hline
\rowcolor{lightgray}   sep1 &  0.1157 &  0.1249 &  0.1629 &  0.1186 &  0.1661 &  0.1717 &  0.1306 &  0.1316 &  0.1405\\ \hline
\rowcolor{lightgray}   sep2 &  0.1754 &  0.1909 &  0.1436 &  0.1869 &  0.1110 &  0.1344 &  0.1786 &  0.1262 &  0.1879\\ \hline
\rowcolor{lightgray}  p-val &  0.0649 &  0.5511 &  0.2565 &  0.4887 &  0.7967 &  0.1115 &  0.5880 &  0.2599 &  0.3930\\ \hline 
\end{tabular}  
\end{table*}

\begin{table*}[t!]
\centering
 \caption{Results of LIL test for GNU C standard library generator.}
 \label{tab:mojkomp_lil_old}
\begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
 \hline 
\rowcolor{lightgray}     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
\rowcolor{lightgray}     tv &  0.0185 &  0.0243 &  0.0242 &  0.0244 &  0.0210 &  0.0220 &  0.0330 &  0.0237 &  0.0221\\ \hline
\rowcolor{lightgray}   sep1 &  0.2593 &  0.1640 &  0.1844 &  0.2573 &  0.2010 &  0.1853 &  0.2882 &  0.4129 &  0.2563\\ \hline
\rowcolor{lightgray}   sep2 &  0.0807 &  0.2133 &  0.2299 &  0.2060 &  0.1839 &  0.2361 &  0.3456 &  0.2078 &  0.1405\\ \hline
\rowcolor{lightgray}  p-val &  0.9627 &  0.4878 &  0.5225 &  0.3022 &  0.6978 &  0.5382 &  0.0009 &  0.4903 &  0.7901\\ \hline
\end{tabular}  
\end{table*}


For our tests we took all 31 bits outputted by PRNG. From the results gathered in Tables \ref{tab:mojkomp_asin}
and \ref{tab:mojkomp_lil} one may conclude that ASIN test gives no reason for rejecting the hypothesis that
the sequences generated by the analyzed PRNG are random. In the case of LIL test, the results for $n=2^{34}$ and $n=2^{33}$
may also suggest that this PRNG is good. But for $n=2^{32}$ we can observe an evident deviation,
namely the $p$-value is very small, only about $1/1000$. This can be a matter of chance -- with probability $1/1000$ this
could happen even for a truly random generator. However, take a look on $p$-values for ten data subsets of size 1000
(\ie each sample consists of 1000 sequences). We have $0.9313$, $0.0949$, $0.8859$, $0.1739$, $0.3675$, $0.0334$, $0.0321$,
$0.1824$, $0.0017$, $0.6205$.  As we can see, 4 out of 10 $p$-values are below $0.1$. The probability that for truly random
sequences at least 4 $p$-values fall into that interval is
\[ 1 - \sum_{i=0}^3 \binom{10}{i} \left(\frac{1}{10}\right)^{i} \left(1 - \frac{1}{10}\right)^{10-i} \approx 0.0016~. \]
This suggests that the GLIBC standard library PRNG may contain some hidden flaws. 
However, despite the issue pointed above, the implementation of \texttt{rand} function considered in this section
appears to be the best among these already tested by us.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Minstd %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Minstd}
Minstd (abbr. from \textit{minimal standard generator}) is based on MCG with parameters recommended by Park and Miller
in \cite{Park1988}. The authors' goal was to develop a simple generator, not necessarily perfect, but fast, simple to
implement and suitable for most common applications. As a result they proposed $MCG(2^{31}-1, 16807)$.
%For generating binary sequences eight most significant bits returned by the PRNG were used.
%The results of experimental testing are shown in Tables \ref{tab:minstd_asin} and \ref{tab:minstd_lil}.
% 
% \begin{table*}[t!]
% \centering
%  \caption{Results of arcsine test for Minstd generator with multiplier 16807.}
%  \label{tab:minstd_asin}
% \begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
%  \hline
%      n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
%      tv &  0.0321 &  0.0321 &  0.0402 &  0.0725 &  0.0917 &  0.1116 &  0.1648 &  0.2003 &  0.2109\\ \hline
%    sep1 &  0.1172 &  0.1686 &  0.1407 &  0.2985 &  0.2880 &  0.6670 &  0.5203 &  0.7345 &  0.8486\\ \hline
%    sep2 &  0.1302 &  0.1490 &  0.2420 &  0.3986 &  0.4051 &  0.3735 &  0.3822 &  0.5352 &  0.3894\\ \hline
%   p-val &  0.0360 &  0.0203 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline
% \end{tabular}  
% \end{table*}
% 
% \begin{table*}[t!]
% \centering
%  \caption{Results of LIL test for Minstd generator with multiplier 16807.}
%  \label{tab:minstd_lil}
% \begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
%  \hline 
%      n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
%      tv &  0.0370 &  0.0622 &  0.0823 &  0.1120 &  0.1877 &  0.2002 &  0.3538 &  0.3194 &  0.9500\\ \hline
%    sep1 &  0.5035 &  0.5465 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
%    sep2 &  0.1444 &  0.2366 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
%   p-val &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline
% \end{tabular}  
% \end{table*}
In their later work from 1993, Park and Miller \cite{Park1993} suggested that it would be better to use 
the multiplier $48271$.
However, changing the multiplier does not affect our tests much. 
In Tables \ref{tab:nminstd_asin} and \ref{tab:nminstd_lil} the results for $48271$ are presented,
and those for $16807$ (not included here) are similar. 
 

\begin{table*}[t!]
\centering
 \caption{Results of ASIN test for Minstd generator with multiplier 48271.}
 \label{tab:nminstd_asin}
\begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
 \hline
     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
     tv &  0.0318 &  0.0430 &  0.0477 &  0.0982 &  0.1303 &  0.0918 &  0.0848 &  0.1131 &  0.2089\\ \hline
   sep1 &  0.1607 &  0.1467 &  0.1901 &  0.3803 &  0.4280 &  0.3845 &  0.4583 &  0.3975 &  0.8079\\ \hline
   sep2 &  0.1828 &  0.1719 &  0.2120 &  0.2548 &  0.3449 &  0.3179 &  0.3192 &  0.3186 &  0.4579\\ \hline
  p-val &  0.0115 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline
\end{tabular}  
\end{table*}

\begin{table*}[t!]
\centering
 \caption{Results of LIL test for Minstd generator with multiplier 48271.}
 \label{tab:nminstd_lil}
\begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
 \hline 
     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
     tv &  0.0372 &  0.0563 &  0.0590 &  0.2573 &  0.2879 &  0.3408 &  0.3167 &  0.3434 &  0.9500\\ \hline
   sep1 &  0.3298 &  0.4839 &  0.9328 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
   sep2 &  0.3843 &  0.1850 &  0.2207 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
  p-val &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline
\end{tabular}  
\end{table*}
For the ASIN tests the total variation distance between theoretical and empirical measures decreased in most cases
after changing the multiplier, especially for longer sequences. But in the case of LIL tests the opposite change occurred. 
Thus, based on these results it is hard to say whether this modification brings significant improvement. Nevertheless,
$\chi^2$ test in both cases shows that Minstd is not a sound PRNG.

Despite its weaknesses, Minstd became a part C++11 standard library. It is implemented by the classes
\texttt{std::minstd\_rand0} (with multiplier 16807) and \texttt{std::minstd\_rand} (with multiplier 48271).


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Mersene Twister %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Mersenne Twister}
Mersenne Twister generator was tested using the built-in implementation in C++11. 
We chose 64-bit version of the PRNG
\ie class \texttt{std::mt19937\_64}. 
%%%It is a minor modification of 32-bit variant characterized in Section \ref{subsec:prng},
%%% adapted to architectures with 8-byte words. 
In tests all 64 bits returned by a single call to the generator were used.
\begin{table*}[t!]
\centering
 \caption{Results of ASIN test for C++11 implementation of MT19937-64 generator.}
 \label{tab:twister_asin}
\begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
 \hline
     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
     tv &  0.0271 &  0.0245 &  0.0226 &  0.0281 &  0.0276 &  0.0228 &  0.0271 &  0.0230 &  0.0255\\ \hline
   sep1 &  0.1421 &  0.1606 &  0.1167 &  0.1824 &  0.1938 &  0.1571 &  0.1760 &  0.1397 &  0.1573\\ \hline
   sep2 &  0.1133 &  0.1195 &  0.1056 &  0.1399 &  0.1256 &  0.1287 &  0.1391 &  0.0994 &  0.1444\\ \hline
  p-val &  0.2755 &  0.6823 &  0.8804 &  0.0801 &  0.1267 &  0.7343 &  0.1094 &  0.7596 &  0.2029\\ \hline
\end{tabular}  
\end{table*}
\begin{table*}[t!]
\centering
 \caption{Results of LIL test for C++11 implementation of MT19937-64 generator.}
 \label{tab:twister_lil}
\begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
 \hline 
     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
     tv &  0.0254 &  0.0264 &  0.0238 &  0.0234 &  0.0266 &  0.0265 &  0.0290 &  0.0299 &  0.0215\\ \hline
   sep1 &  0.1853 &  0.2147 &  0.1689 &  0.3093 &  0.1887 &  0.2015 &  0.2877 &  0.2318 &  0.1953\\ \hline
   sep2 &  0.2841 &  0.1696 &  0.1917 &  0.1282 &  0.2017 &  0.2492 &  0.1842 &  0.1541 &  0.1716\\ \hline
  p-val &  0.2483 &  0.3690 &  0.5965 &  0.5066 &  0.2196 &  0.1495 &  0.0499 &  0.0189 &  0.8170\\ \hline
\end{tabular}  
\end{table*}


\begin{table*}[t!]
\centering
 \caption{Results of arcsine test for C++11 implementation of MT19937-64 generator. \textsc{Time: 18549m53.924s}}
 \label{tab:twister_asin_old}
\begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
 \hline
\rowcolor{lightgray}     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
\rowcolor{lightgray}     tv &  0.0272 & 0.0245 & 0.0226 & 0.0279 & 0.0273 & 0.0223 & 0.0273 & 0.0233 & 0.0252\\ \hline
\rowcolor{lightgray}   sep1 &  0.1421 & 0.1666 & 0.1167 & 0.1824 & 0.1938 & 0.1571 & 0.1760 & 0.1397 & 0.1573\\ \hline
\rowcolor{lightgray}   sep2 &  0.1133 & 0.1195 & 0.1056 & 0.1399 & 0.1209 & 0.1315 & 0.1391 & 0.1065 & 0.1444\\ \hline
\rowcolor{lightgray}  p-val &  0.2548 & 0.6674 & 0.8907 & 0.1014 & 0.1287 & 0.7727 & 0.1002 & 0.7447 & 0.2523\\ \hline
\end{tabular}  
\end{table*}

\begin{table*}[t!]
\centering
 \caption{Results of LIL test for C++11 implementation of MT19937-64 generator. \textsc{Time: 17491m26.914s}}
 \label{tab:twister_lil_old}
\begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
 \hline 
\rowcolor{lightgray}     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
\rowcolor{lightgray}     tv &  0.0229 & 0.0243 & 0.0234 & 0.0207 & 0.0251 & 0.0297 & 0.0287 & 0.0309 & 0.0225\\ \hline
\rowcolor{lightgray}   sep1 &  0.1606 & 0.2400 & 0.1689 & 0.2890 & 0.1458 & 0.1853 & 0.2712 & 0.2318 & 0.1795\\ \hline
\rowcolor{lightgray}   sep2 &  0.2106 & 0.1458 & 0.2017 & 0.1228 & 0.1839 & 0.2492 & 0.1951 & 0.1748 & 0.1559\\ \hline
\rowcolor{lightgray}  p-val &  0.5440 & 0.6035 & 0.4630 & 0.8106 & 0.4609 & 0.0653 & 0.0593 & 0.0077 & 0.7745\\ \hline
\end{tabular}  
\end{table*}



The results presented in Tables \ref{tab:twister_asin} and \ref{tab:twister_lil} give an explanation 
why the Mersenne Twister is one of the most popular PRNG used in practice. These outcomes 
give no arguments against the claim that the output of this PRNG is indeed truly random. 
\medskip\par 
It is worth noting that the experiments for CMRG (not included here) gave similar results. 
Nevertheless, one should note that in \cite{Kim2008} 
the authors provide strong evidence that the output of CMRG is not sound.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Hypothetical flawed PRNG %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Hypothetical flawed PRNG}
\label{subsec:experiments_flawed}
Describing NIST SP800-22 Test Suite in Section  \ref{sec:intro} we pointed out some of its inherent limitations
directly related to the approach applied for statistical testing. Namely, this test suite focuses only on the quality
of single binary sequences produced by PRNGs and does not take into account the set of all bit strings
as a whole. Let us consider some hypothetical PRNG which usually generates sequences which look random, but 
with some non-negligible probability (e.g., for some subset of seeds) its output is biased and far from truly random.
Such flawed sequence will be surely recognized by NIST Test Suite as non-random, but this deviation probably will not cause
considering whole PRNG as ``not good''. However, its output will be easily distinguishable from uniform bit strings.
This issue was carefully discussed in Section 3 in \cite{Wang2015}, where some specific examples of such PRNGs were presented.

The following example gives an insight how this kind of weaknesses in generator's output will be detected by the
discussed distance based tests, \ie LIL test and ASIN test. We will consider the following PRNG. 
\par 
%\textcolor{red}{PL: nie chcielismy tutaj od razu napisac, ze de facto to tylko arcus sinus tes wykrywa?}
\begin{itemize}
	\item For one in every hundred seeds it returns the sequence described by the regular expression 10(0110)*01,
	      \ie binary string starting with 10, followed by repeated runs of 0110 and ending with 01. 
	\item Otherwise, the the output of MT19937-64 generator is returned.
\end{itemize}

\begin{table*}[t!]
\centering
 \caption{Results of ASIN test for the flawed generator described in Section \ref{subsec:experiments_flawed}.}
 \label{tab:zep_asin}
\begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
 \hline
     n  &  $2^{20}$ &  $2^{21}$ &  $2^{22}$ &  $2^{23}$ &  $2^{24}$ &  $2^{25}$ &  $2^{26}$ &  $2^{27}$ &  $2^{28}$\\ \hline
     tv &  0.0326 &  0.0241 &  0.0281 &  0.0285 &  0.0298 &  0.0339 &  0.0298 &  0.0285 &  0.0276\\ \hline
   sep1 &  0.1466 &  0.1754 &  0.1529 &  0.1124 &  0.1249 &  0.1752 &  0.1594 &  0.1666 &  0.1257\\ \hline
   sep2 &  0.3255 &   0.334 &   0.345 &  0.4212 &  0.3608 &  0.3582 &  0.3556 &  0.3925 &  0.3901\\ \hline
  p-val &  0.0000 &  0.0031 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline
\end{tabular}  
\end{table*}

\begin{table*}[t!]
\centering
 \caption{Results of LIL test for the flawed generator described in Section \ref{subsec:experiments_flawed}.}
 \label{tab:zep_lil}
\begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
 \hline 
     n  &  $2^{20}$ &  $2^{21}$ &  $2^{22}$ &  $2^{23}$ &  $2^{24}$ &  $2^{25}$ &  $2^{26}$ &  $2^{27}$ &  $2^{28}$\\ \hline
     tv &  0.0239 &  0.0303 &  0.0255 &  0.0269 &  0.0241 &  0.0280 &  0.0248 &  0.0294 &  0.0229\\ \hline
   sep1 &  0.1929 &  0.2834 &  0.1541 &  0.2018 &  0.2327 &  0.1586 &  0.1631 &  0.2654 &  0.1689\\ \hline
   sep2 &  0.1625 &  0.1517 &  0.1663 &  0.1469 &  0.1381 &  0.1648 &  0.2106 &  0.1667 &  0.1815\\ \hline
  p-val &  0.4073 &  0.0199 &  0.2584 &  0.1250 &  0.5742 &  0.1250 &  0.2703 &  0.0436 &  0.5789\\ \hline
\end{tabular}  
\end{table*}

Testing results for this PRNG are shown in Tables \ref{tab:zep_asin} and \ref{tab:zep_lil}. The outcomes of ASIN test
clearly indicate that the generator is flawed and its output cannot be recognized as random. What is interesting, however,
this is not the case for LIL test, where the obtained $p$-values give no sufficient evidence for rejecting this PRNG.
The reason behind the differences in the behavior of ASIN and LIL tests is that the trajectory of
(surely non-)random walk described by
pattern 10(0110)*01 resembles a triangle wave oscillating around the 0-axis. Therefore, the fraction of time when number of 1s
exceeds number of 0s (\ie the random walk is above 0-axis) is exactly $\frac{1}{2}$. Hence, the value of characteristic
$\Sasin{n}$ falls into the least probable interval in the partition $\mathcal{P}^{asin}$ in almost $0.01\cdot m$ trials more
than for uniform bit sequences. This suffices for significant increase of the value of statistic \label{eq:chi_asin}.
On the other hand, the characteristic $\Slil{n}$ takes for this sequence value 0 belonging to the most likely interval
in the partition $\mathcal{P}^{lil}$. Thus, it is more difficult for $\chi^2$ test to detect such deviation. Nevertheless,
if we use e.g. $m=100000$ sequences in the experiments above, LIL based test will also identify this weakness of considered
generator. This leads to the conclusion that in order to detect such kinds of flaws in PRNGs implementations one should
increase the number of sequences tested rather than the length of individual binary string.

% \textcolor{blue}{
We also performed \texttt{TestU01} on our flawed generator (including $J$ 
statistic from \texttt{swalk}).
The results were similar to ours - in all the cases (different sequences' 
length) the corresponding $p$-value for statistic $J$ was 0.0 . The size of 
the partion was automatically set to 998 (whereas we used $s=40$). 
We also performed tests from NIST Test Suite - the flawed generator passed many of them, details given in next section.
% }


%Dlaczego w tym wypadku test iterowanego logarytmu się nie sprawdził? Błądzenie (zdecydowanie nieprzypadkowe) opisane wyrażeniem $10(0110)^*01$ oscyluje wokół osi OX jak sinusoida. Oznacza to, że frakcja czasu przewagi liczby jedynek nad liczbą zer jest równa dokładnie $\frac{1}{2}$. Dzięki temu wartość charakterystyki $\Sasin{n}$ wpada do najmniej prawdopodobnego przedziału w partycji $\mathcal{P}^{asin}$ w prawie $0.01m$ przypadkach częściej niż dla dobrego generatora. Wystarcza to by wartość statystyki (\ref{eq:chi_asin}) bardzo urosła. Tymczasem charakterystyka $\Slil{n}$ przyjmuje dla ciągu $10(0110)^*01$ wartość zero, a tym samym wpada do najbardziej prawdopodobnego przedziału. Dlatego testowi $\chi^2$ trudniej jest to wykryć.
%
%Gdybyśmy jednak w powyższym eksperymencie wykorzystali $m = 100000$ ciągów, to również test iterowanego logarytmu zauważyłby zbyt duże odstępstwo. Wypływa stąd wniosek, że w celu wykrywania tego rodzaju wad generatorów lepiej postawić na liczbę ciągów, a nie na ich długość.

\subsubsection{NIST Test Suite}

For  $m=10000$ sequences of length 
$n=2^{15}$, the ASIN test already returns $p$-value 0.000.
For comparison, for this parameters we ran  
we ran a battery NIST Test Suite. 
Results are given in Table \ref{tab:flaw_nist}.
For each sequence the corresponding $p$-value is was calculated. 
NIST adopted two ways to interpret a set of $p$-values: a) examination of proportion of sequences that pass 
a certain test; b) testing the uniformity of $p$-values (for truly random sequences they should be 
uniformly distributed in $[0,1]$). 
\par 
Values in the columns C1,$\ldots,$ C10 represent number of $p$-values falling into intervals 
$[0.0, 0.1), [0.1,0.2),\ldots,[0.9,1]$. Values in P-VALUE column represent the results for uniformity testing 
of $p$-values, value in PROPORTION column represent proportion of sequences that pass a given test.
The character $*$ denotes that the PRNG failed given test (more exactly: given interpretation of a set of $p$-values).
For detailed description of results' interpretation see \cite{Rukhin2010}.
Note that some tests from NIST Test Suite detected the flaw, but most did not.

\begin{table*}[t!]
\scriptsize
\centering
 \caption{Partial results from the \texttt{finalAnalysisReport.txt} file produced by NIST Test Suite 
 applied for $10^4$ sequences of length $2^{15}$ of flawed generator.}\label{tab:flaw_nist}.
 \begin{tabular} {|p{0.5cm}|p{0.5cm}|c|c|c|c|c|c|c|c|l|l|c|c|c|c|c|c|c|c|}   
 \hline 
% ------------------------------------------------------------------------------                                                                                                       
%  C1  C2  C3  C4  C5  C6  C7  C8  C9 C10  P-VALUE  PROPORTION  STATISTICAL TEST       

% ------------------------------------------------------------------------------                                                                                                       
% 987 1036 980 961 1099 798 925 981 993 1240  0.000000 * 9896/10000    Frequency                                                                                                       
% 990 1013 949 981 1013 1011 996 987 1007 1053  0.682410   9898/10000    BlockFrequency                                                                                                
% 985 964 894 1120 889 832 1084 902 1117 1213  0.000000 * 9889/10000    CumulativeSums                                                                                                 
% 1010 996 857 1100 868 829 1158 875 1051 1256  0.000000 * 9892/10000    CumulativeSums                                                                                                
% 947 998 948 921 1001 1009 974 1079 1065 1058  0.001793   9910/10000    Runs                                                                                                          
% 1119 992 1026 964 936 1081 1002 925 987 968  0.000102   9794/10000 *  LongestRun                                                                                                     
% 1502   0 2865   0   0   0 5633   0   0   0  0.000000 * 10000/10000 *  Rank                                                                                                           
% 1040 1111 518 1366 1753   0 2015   0 1107 1090  0.000000 * 9791/10000 *  FFT  
C1& C2 & C3 & C4 & C5 & C6 & C7 & C8 & C9 & C10 &  \tiny P-VALUE & \tiny PROPORTION & \tiny STATISTICAL TEST       \\\hline
% 987& 1036 & 980 & 961 & 1099 & 798 & 925 & 981 & 993 & 1240 & 0.000000  * & 9896/10000 &  Frequency \\
% 990& 1013 & 949 & 981 & 1013 & 1011 & 996 & 987 & 1007 & 1053 & 0.682410 & 9898/10000 & BlockFrequency \\
% 985& 964 & 894 & 1120 & 889 & 832 & 1084 & 902 & 1117 & 1213 & 0.000000  * & 9889/10000 & CumulativeSums \\ 
% 1010& 996 & 857 & 1100 & 868 & 829 & 1158 & 875 & 1051 & 1256 & 0.000000  * & 9892/10000 & CumulativeSums \\
% 947& 998 & 948 & 921 & 1001 & 1009 & 974 & 1079 & 1065 & 1058 & 0.001793 & 9910/10000 & Runs  \\
% 1119& 992 & 1026 & 964 & 936 & 1081 & 1002 & 925 & 987 & 968 & 0.000102 &  9794/10000  * & LongestRun \\
% 1502& 0 & 2865 & 0 & 0 & 0 & 5633 & 0 & 0 & 0 & 0.000000  * & 10000/10000 * & Rank  \\
% 1040& 1111 & 518 & 1366 & 1753 & 0 & 2015 & 0 & 1107 & 1090 & 0.000000  * & 9791/10000  * & FFT \\\hline

976 & 1043 & 972 & 1007 & 943 & 1053 & 1029 & 960 & 924 & 1093 & 0.001907 & 9907/10000 & Frequency \\
1015 & 999 & 927 & 972 & 1015 & 971 & 991 & 983 & 1029 & 1098 & 0.032705 & 9905/10000 & BlockFrequency \\
956 & 982 & 1066 & 996 & 928 & 1028 & 1005 & 996 & 956 & 1087 & 0.008428 & 9901/10000 & CumulativeSums \\
987 & 1027 & 951 & 967 & 1052 & 950 & 1011 & 977 & 938 & 1140 & 0.000101 & 9918/10000 & CumulativeSums\\ 
1042 & 930 & 972 & 1008 & 997 & 986 & 993 & 995 & 957 & 1120 & 0.004239 & 9886/10000 & Runs \\
1013 & 1015 & 1037 & 1014 & 1001 & 1008 & 947 & 988 & 989 & 988 & 0.812723 & 9809/10000  * & LongestRun \\
1006 & 869 & 1136 & 1016 & 1262 & 671 & 1466 & 864 & 778 & 932 & 0.000000  * & 9803/10000  * & Rank \\
1146 & 928 & 987 & 1055 & 868 & 995 & 1076 & 949 & 993 & 1003 & 0.000000  * & 9778/10000  * & FFT \\
1078 & 939 & 1008 & 999 & 1048 & 1027 & 978 & 1006 & 976 & 941 & 0.041709 & 9787/10000  * & OverlappingTemplate\\
%10000 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0.000000 * &   0/10000  * & Universal\\
2017 & 1305 & 1154 & 1083 & 969 & 911 & 755 & 700 & 596 & 510 & 0.000000  * & 9576/10000  * & ApproximateEntropy\\
 5 & 9 & 2 & 6 & 6 & 3 & 5 & 4 & 6 & 8 & 0.494392 & 53/54 & RandomExcursions\\
 6 & 4 & 5 & 4 & 6 & 5 & 7 & 4 & 6 & 7 & 0.971699 & 54/54 & RandomExcursions\\
 9 & 5 & 2 & 1 & 5 & 6 & 4 & 8 & 4 & 10 & 0.075719 & 54/54 & RandomExcursions\\
11 & 4 & 7 & 3 & 6 & 6 & 2 & 5 & 9 & 1 & 0.040108 & 51/54 & RandomExcursionsVariant\\
 10 & 6 & 5 & 3 & 5 & 5 & 2 & 7 & 6 & 5 & 0.455937 & 53/54 & RandomExcursionsVariant\\
 8 & 9 & 4 & 1 & 6 & 6 & 7 & 4 & 5 & 4 & 0.350485 & 53/54 & RandomExcursionsVariant\\
 9 & 8 & 3 & 1 & 10 & 9 & 4 & 2 & 6 & 2 & 0.011791 & 53/54 & RandomExcursionsVariant\\
1201 & 935 & 1038 & 983 & 1005 & 949 & 971 & 951 & 978 & 989 & 0.000000  * & 9682/10000  * & Serial\\
1214 & 980 & 1037 & 1013 & 886 & 1001 & 934 & 925 & 1025 & 985 & 0.000000  * & 9697/10000  * & Serial\\
1112 & 875 & 931 & 933 & 1038 & 1057 & 1057 & 1073 & 966 & 958 & 0.000000  * & 9731/10000  * & LinearComplexity\\\hline 
\end{tabular}
\begin{flushleft}
 
- - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\par \noindent
\texttt{The minimum pass rate for each statistical test with the exception of the
random excursion (variant) test is approximately = 9870 for a
sample size = 10000 binary sequences.
}
\medskip\par \noindent
\par\texttt{The minimum pass rate for the random excursion (variant) test
is approximately = 51 for a sample size = 54 binary sequences.} \par
- - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -

\end{flushleft}

\end{table*}


==> sections/experiments_oo.tex <==
% 4.1. BSD libc rand() -> "Rand"
% 4.2. Microsoft Visual C++ rand() -> "SVIS"
% 4.3. GLIBC stdlib rand() -> "C_PRG"
% 4.4. Minstd with multiplier 48271 -> "NewMinstd3"
% 4.5. Mersenne Twister - wbudowana implementacja C++11 -> "Mersenne"
% 4.6. Flawed -> "zepsuty"
%
%


 


In this section we shortly report  experimental results of testing some
widely used PRNGs implemented in standard libraries in various programming languages.
We performed  ASIN   test  on generators including different implementations
of standard C/C++ linear congruential generators, the standard generator \textsc{rand} from
GNU C Library, Mersenne Twister, Minstd and CMRG generators.  
% Tables present results only for the generators which behave differently.
% \textcolor{red}{tutaj jakos opisac, ze niektorych nie ma w tabelkach bo maja ``same tendency''}
As our last example we propose some hypothetical weak PRNG which is clearly identified
by our ASIN test as non-random, whereas \pl{other 
tests fail to detect its obvious flaw (CZY TO PRAWDA?)}


is the expected 
statistical deviation of the ratio of $p_j$ values found in a given bin.

Each considered PRNG was tested by generating $m = 10000$ sequences of length $n   = 2^{34}$,
with partition $\mathcal{P}_{40}$, \ie $s=40$. 
For these parameters our second level test is reliable (see Section \ref{sec:err_analysis_reliability}):
$\sigma$, the expected statistical deviation of the ratio of $p_j$ values found in a given bin  is greater 
than $\sqrt{ {s-1\over s^2 m}} = 0.0015$  what significantly exceeds the maximum propagated error  
$\Delta={2C\over n}=7.0703 \cdot 10^{-8}$, 
\ie (\ref{eq:Delta_bound}) holds. Note that for $n=2^{34}$ and $s=40$ inequality (\ref{eq:m_bound}) yields 
$m\leq 1.9054 \cdot 10^{13}$.

\pl{Poniewaz nie wiem co bedzie niezbedne, podaje dla pozostalych $n$: 
dla $n=2^{26}$ mamy $\Delta=0.000018$, $m\leq 2.9761\cdot 10^8$ } \par 
\pl{dla $n=2^{30}$ mamy $\Delta = 0.00000113, m\leq 7.6188\cdot 10^{10}$}

% 
% 
% in most cases. The values of characteristics $\Sasin{r}$ or $\Slil{r}$
% were calculated both for each sequence ($r=n$) as well as for subsequences of length $n/2, \ldots, n/2^{k}$
% for some fixed value of $k$ depending on tested PRNG (usually $k = 8$). This approach,
% called in \cite{Wang2015} \emph{snapshot testing} at points $2^{n}, \ldots, 2^{n/2^{k}}$, allows for
% observing and comparing the values of analyzed parameters on different stages.
% Finally, for each PRNG respective statistics and distances between theoretical and empirical distributions
% were calculated, as described in detail in Sections \ref{subsec:arcsineTests} and \ref{subsec:lilTests}.
% In our experimental analysis for tests based on characteristics $\Sasin{n}$ and $\Slil{n}$
% we used partitions $\mathcal{I}^{asin}_{40}$ and $\mathcal{I}^{lil}_{40}$, respectively.
%
In  experiments we used our own implementations of tested PRNGs (except Mersenne Twister).
We used  64-bit version C++11 implementation of  Mersenne Twister,
\ie the class  \texttt{std::mt19937\_64}, 
which is known to have some problems \cite{Harase2017}.
The generators were initialized with random seeds from \url{http://www.random.org} \cite{RandomOrg}
and each sequence was generated using different seed.

\smallskip\par


\begin{table*}[t!]
\centering
 \caption{Results of ASIN test for  several generators with parameters $m=10000, n =2^{34}, s=40$. 
 Bolded values indicate that we reject $\mathcal{H}_0$ with significance level $\alpha=0.0001$.}
 %\textcolor{red}{NewMinstd3 sie robi! jak nie zdazy, damy $2^26$}
 \label{tab:res_all}
\begin{tabular} {|l|c|c|c|c|c|c|c|c|c|c|c|}   
 \hline
   & $d^{asin}_{tv} $ & $p_{\chi^2}$ \\ \hline 
 MS Visual C++ & \textbf{0.2093} & \textbf{0.0000} \\ \hline 
 GNU C & 0.0255 & 0.2389 \\ \hline 
 Minstd 48271 & \textbf{0.2089} & \textbf{0.0000} \\ \hline 
 MT19937-64  & 0.0252 & 0.2523 \\ \hline 
%  
%      n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
%      tv &  0.0318 &  0.0430 &  0.0477 &  0.0982 &  0.1303 &  0.0918 &  0.0848 &  0.1131 &  0.2089\\ \hline
%    sep1 &  0.1607 &  0.1467 &  0.1901 &  0.3803 &  0.4280 &  0.3845 &  0.4583 &  0.3975 &  0.8079\\ \hline
%    sep2 &  0.1828 &  0.1719 &  0.2120 &  0.2548 &  0.3449 &  0.3179 &  0.3192 &  0.3186 &  0.4579\\ \hline
%   p-val &  0.0115 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline
 \end{tabular}  
\end{table*}

\smallskip\par
The results are presented in Table \ref{tab:res_all}. The values indicating that $\mathcal{H}_0$ should be rejected 
(w.r.t. significance level $\alpha=0.0001$, a value suggested by NIST for second level test)
are \textbf{bolded}. For $p_{\chi^2}$ these are simply values smaller or equal to $\alpha$.
Concerning the values of $d^{asin}_{tv} $, Lemma \ref{lem:devroy} implies that for $\varepsilon\leq \sqrt{20\cdot 41/10000}\leq 0.2862$ we 
have $\Pro{d_{tv}^{asin}>{\varepsilon/2}}\leq 3 \exp\left(-400\varepsilon^2\right).$
It can be checked that $3exp(-400\varepsilon^2)\leq 0.0001$ for $\varepsilon\leq 0.1605$, in other words 
$$ \Pro{d_{tv}^{asin}>0.0802}\leq 0.0001,$$
% It can be checked that $3exp(-400\varepsilon^2)\leq 0.01$ for $\varepsilon\leq 0.1194$, in other words 
% $$ \Pro{d_{tv}^{asin}>0.0597}\leq 0.01,$$
\ie we reject $\mathcal{H}_0$ if the value of $d_{tv}^{asin}$ is larger than $0.0802$.
Note that for results in Table \ref{tab:res_all} either both statistics $d_{tv}^{asin}$
and $p$-value of $T^{asin}$ reject $\mathcal{H}_0$ 
or both accept it.

% \textcolor{red}{UWAGA: chyba w second level test NIST zaleca (tzn. on robi dla roznych testow..),
% by w drugim poziomie uzyc $\alpha=0.0001$... wtedy mamy 
%  $3 \exp\left(-400\varepsilon^2\right)=0.0001$ dla $\varepsilon = 0.1605$ i wtedy 
%  $$ \Pro{d_{tv}^{asin}>0.0802}\leq 0.0001,$$ ... w tabelce ok, te same zdaja/nie zdaja.
%  ZMIENIC? (wtedy tez w Introduction)}
% 


\smallskip\par
We also calculated \texttt{swalk\_RandomWalk1} statistics   from \texttt{TestU01} for 
 10000 sequences of length $2^{26}$ of each  PRNG.
 The following parameters for \texttt{swalk\_RandomWalk1}  were used: $N=1, 
n=10000, r=0, s=32, L0=L1=67108864 = 2^{26}$.  The result are given in Table 
\ref{tab:tesu01_all} (including \textsl{Flawed} generator described in Section 
\ref{subsec:experiments_flawed}).  For each Statistic H, M, J, R and C $p$-values were 
obtained using
 \textsl{chi-square}
statistics.
 For convenience, $p$-values of $T^{asin}$ are  also   included in the 
Table~\ref{tab:tesu01_all}.



\begin{table*}[t!]
\centering \small
 \caption{Results ($p$-values) of $T^{asin}$ and \texttt{swalk\_RandomWalk1} statistics from \texttt{TestU01} for $n=2^{26}$
(for parameters [\texttt{TestU01} notation]: $N =  1,  n = 10000,  r =  0,   s = 32,   L0 = L1 = 2^{26}$). Bolded values 
indicate that we reject $\mathcal{H}_0$ with significance level $\alpha=0.01$.}
 \label{tab:tesu01_all}
\begin{tabular} {|l|c|c|l|l|l|l|l|c|c|c|c|}   
 \hline
    PRNG\textbackslash Test &  $p_{\chi^2}$ 	&  Statistic  H  	
&  Statistic  M 		&  Statistic  J  	&  Statistic  R 	 
  &  Statistic  C  \\ \hline
%     BSD libc     &  0.0000 	& \quad 0.0000  &  
%\quad 0.0000	 & \quad 0.0000  & \quad 0.0000  & \quad 0.0000	  \\ \hline
		
	
MS Visual C++   &  0.0148 	& \quad 0.2700 & \quad 0.0900	 & 
\quad 0.6300  & \quad 0.4200 & \quad 0.8000 \\ \hline
	
	
	
      GNU C   &   0.4731		& \quad 0.1600 &  
\quad 0.9800	 & \quad 0.1100  & \quad 0.1900  & \quad 0.4900 \\ \hline

		
   Minstd 48271	  &  0.0115 			& \quad \textbf{0.0090} & 
 \quad 0.1400 & \quad 0.4900 & \quad 0.0700 &	\quad \textbf{0.0044} \\ \hline
		
   MT19937-64 	  &  0.2548 	 		& \quad 0.0800 &  
\quad 0.1000 & \quad 0.4200 & \quad 0.9700 &	\quad 0.3500 \\  \hline

$\textsf{Flawed}_{\rm MT19937-64, 26, 1/66} $ &  \textbf{0.0000}			& \quad \textbf{0.0000} &  
\quad 0.2200 & \quad \textbf{0.0000} & \quad 0.3900&	\quad 0.3800 \\  \hline

		
\end{tabular}  
\end{table*}

\pl{w TAble \ref{tab:tesu01_all} dopisalem parametry flawed $\textsf{Flawed}_{\rm MT19937-64, 26, 1/66} $ UWAGA:  
wyniki w TAble \ref{tab:tesu01_all}  sa juz nowe dla tau=1/66 z 18.11.15 }
\par 
\pl{Flawed chyba jest roznymi czcionkami w roznych miejscach ... }

\medskip\par 
Our ASIN test would reject MS Visual C++ PRNG and Minstd with multiplier 48271
(Minstd with multiplier 16807 gave similar results - not reported here) as 
good PRNGs. Note that both, $p_{\chi^2}$ and the value of $d_{tv}^{asin}$ 
indicate it. We also conducted (not included here) the experiments 
for  the procedure \texttt{rand} from a standard library in Borland C/C++.
The outcomes are very akin to those for a standard PRNG in MS Visual C++.
Note  that for  $n=2^{26}$ none of the  $p$-values of 
\texttt{swalk\_RandomWalk1} from \texttt{TestU01} suggests rejecting
the hypothesis that MS Visual C++ PRNG is good, 
whereas statistics H and C indicate that there can be 
some flaws in Minstd 48271. 
It is worth mentioning that MS Visual C++ PRNG passes the NIST Test Suite \cite{NISTtests}, as pointed out in \cite{Wang2015}.
Minstd, despite its weaknesses, became a part C++11 standard library
It is implemented by the classes
\texttt{std::minstd\_rand0} (with multiplier 16807) and \texttt{std::minstd\_rand} (with multiplier 48271).
 
 
Concerning GNU C and MT19937-64 -- as can be seen in both Table 
\ref{tab:res_all} and Table \ref{tab:tesu01_all} --  can be considered as good.
It is worth mentioning that results (not reported here) 
for CMRG generator were similar to those for  MT19937-64.

The open source code of our implementation is available, see 
\cite{ArcsineTest_github} (it includes the \textsl{Flawed} PRNG described below).



\input{sections/flawed_chi2.tex}

\paragraph{Results of ASIN and LIL tests for \textsl{Flawed}} 


\begin{table*}[t!]
\centering
 \caption{Results of ASIN test for the \textsl{Flawed} generator described in Section \ref{subsec:experiments_flawed}. \texttt{Time: 83 min 59s}}
 \label{tab:zep_asin}
\begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
 \hline
     n  &  $2^{19}$ & $2^{20}$ &  $2^{21}$ &  $2^{22}$ &  $2^{23}$ &  $2^{24}$ &  $2^{25}$ &  $2^{26}$\\ \hline
     tv &  0.0222 & 0.0301 & 0.0213 & 0.0232 & 0.0230 & 0.0258 & 0.0296 & 0.0301\\ \hline
   sep1 &  0.1011 & 0.1529 & 0.1754 & 0.1305 & 0.1029 & 0.1186 & 0.1567 & 0.1594\\ \hline
   sep2 &  0.1022 & 0.1635 & 0.1256 & 0.1404 & 0.1348 & 0.1709 & 0.1536 & 0.3582\\ \hline
  p-val &  0.9401 & 0.0567 & 0.8188 & 0.4730 & 0.7640 & 0.3532 & 0.0498 & 0.0000\\ \hline
\end{tabular}  
\end{table*}
\begin{table*}[t!]
\centering
 \caption{Results of LIL test for the \textsl{Flawed} generator described in Section \ref{subsec:experiments_flawed}. \texttt{Time: 77 min 46 s}}
 \label{tab:zep_lil}
\begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
 \hline 
     n  &  $2^{19}$ & $2^{20}$ &  $2^{21}$ &  $2^{22}$ &  $2^{23}$ &  $2^{24}$ &  $2^{25}$ &  $2^{26}$\\ \hline
     tv &  0.0203 & 0.0192 & 0.0260 & 0.0212 & 0.0233 & 0.0208 & 0.0276 & 0.023\\ \hline
   sep1 &  0.2047 & 0.1929 & 0.2834 & 0.1541 & 0.2018 & 0.2327 & 0.1586 & 0.1631\\ \hline
   sep2 &  0.2309 & 0.0998 & 0.1459 & 0.1663 & 0.1299 & 0.1381 & 0.1648 & 0.2106\\ \hline
  p-val &  0.7220 & 0.9829 & 0.2290 & 0.9229 & 0.5943 & 0.8944 & 0.1497 & 0.5558\\ \hline
\end{tabular}  
\end{table*}




% 
% \begin{table*}[t!]
% \centering
%  \caption{Results of ASIN test for the flawed generator described in Section \ref{subsec:experiments_flawed}. \textcolor{red}{to stary Grzeska flawed - wywalamy czy zost?}}
%  \label{tab:zep_asin_old}
% \begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
%  \hline
% \rowcolor{lightgray}     n  &  $2^{20}$ &  $2^{21}$ &  $2^{22}$ &  $2^{23}$ &  $2^{24}$ &  $2^{25}$ &  $2^{26}$ &  $2^{27}$ &  $2^{28}$\\ \hline
% \rowcolor{lightgray}     tv &  0.0326 &  0.0241 &  0.0281 &  0.0285 &  0.0298 &  0.0339 &  0.0298 &  0.0285 &  0.0276\\ \hline
% \rowcolor{lightgray}   sep1 &  0.1466 &  0.1754 &  0.1529 &  0.1124 &  0.1249 &  0.1752 &  0.1594 &  0.1666 &  0.1257\\ \hline
% \rowcolor{lightgray}   sep2 &  0.3255 &   0.334 &   0.345 &  0.4212 &  0.3608 &  0.3582 &  0.3556 &  0.3925 &  0.3901\\ \hline
% \rowcolor{lightgray}  p-val &  0.0000 &  0.0031 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline
% \end{tabular}  
% \end{table*}
% 
% \begin{table*}[t!]
% \centering
%  \caption{Results of LIL test for the flawed generator described in Section \ref{subsec:experiments_flawed}. \textcolor{red}{to stary Grzeska flawed - wywalamy czy zost?}}
%  \label{tab:zep_lil_old}
% \begin{tabular} {|c|c|c|c|c|c|c|c|c|c|c|c|}   
%  \hline 
% \rowcolor{lightgray}     n  &  $2^{20}$ &  $2^{21}$ &  $2^{22}$ &  $2^{23}$ &  $2^{24}$ &  $2^{25}$ &  $2^{26}$ &  $2^{27}$ &  $2^{28}$\\ \hline
% \rowcolor{lightgray}     tv &  0.0239 &  0.0303 &  0.0255 &  0.0269 &  0.0241 &  0.0280 &  0.0248 &  0.0294 &  0.0229\\ \hline
% \rowcolor{lightgray}   sep1 &  0.1929 &  0.2834 &  0.1541 &  0.2018 &  0.2327 &  0.1586 &  0.1631 &  0.2654 &  0.1689\\ \hline
% \rowcolor{lightgray}   sep2 &  0.1625 &  0.1517 &  0.1663 &  0.1469 &  0.1381 &  0.1648 &  0.2106 &  0.1667 &  0.1815\\ \hline
% \rowcolor{lightgray}  p-val &  0.4073 &  0.0199 &  0.2584 &  0.1250 &  0.5742 &  0.1250 &  0.2703 &  0.0436 &  0.5789\\ \hline
% \end{tabular}  
% \end{table*}
 
Testing results for this PRNG which produced $m=10000$ sequences of length $2^{26}$ are shown in Tables \ref{tab:zep_asin} and \ref{tab:zep_lil}. 
As we expected, for $n=2^{26}$ the outcome of ASIN test
clearly indicates that the generator is flawed and its output cannot be recognized as random.
\textcolor{red}{UWAGA: te tabelki do zmiany... nie ma juz sep1, sep2... zob. jak sie zmienily poprzednie 
tabelki. Nie mamy tez testu LIL, moze mozna napisac, ze ``Not reported''}
Note that 
this is not the case for LIL test, where the obtained $p$-values give no sufficient evidence for rejecting this PRNG.
The reason behind the differences in the behavior of ASIN and LIL tests is that  every hundredth  trajectory
of \textsl{Flawed} is exactly half of the time above $x$-axis, and half of the time below it.
Therefore, the fraction of time when number of 1s
exceeds number of 0s (\ie the random walk is above $x$-axis) is exactly $\frac{1}{2}$. Hence, the value of characteristic
$\Sasin{n}$ falls into the least probable interval in the partition $\mathcal{P}_40$ in almost $0.01\cdot m$ trials more
than for uniform bit sequences. This suffices for significant increase of the value of statistic \label{eq:chi_asin}. 


On the other hand, the characteristic $\Slil{n}$ takes values which belong to very likely intervals in the partition $\mathcal{P}^{lil}$
(first quarter of bits are from MT19937-64, then the walk is forced (however randomly) to go to 0 in the middle, then
oscillates around zero in a similar way as in the first half). Thus, it is more difficult for $\chi^2$ test to detect such deviation. 

Note also that only Statistic J of \texttt{swalk\_RandomWalk1} from \texttt{TestU01}  is able to detect this flaw,   see Table \ref{tab:tesu01_all}.
The $p$-values of LIL and Statistic M  for  \textsl{Flawed} are even ``better''  than the ones for Mersenne Twister. 
At first glance it may be surprising, since
\textsl{Flawed} is strongly based on Mersenne Twister (and is non-random). But this is because - in a sense - 
a walk (randomly enough, but) ``oscillates'' around $x$-axis and tests similar to LIL cannot detect such flaws.


% Nevertheless,
% if we use e.g. $m=100000$ sequences in the experiments above, LIL based test will also identify this weakness of considered
% generator. This leads to the conclusion that in order to detect such kinds of flaws in PRNGs implementations one should
% increase the number of sequences tested rather than the length of individual binary string.




%Dlaczego w tym wypadku test iterowanego logarytmu się nie sprawdził? Błądzenie (zdecydowanie nieprzypadkowe) opisane wyrażeniem $10(0110)^*01$ oscyluje wokół osi OX jak sinusoida. Oznacza to, że frakcja czasu przewagi liczby jedynek nad liczbą zer jest równa dokładnie $\frac{1}{2}$. Dzięki temu wartość charakterystyki $\Sasin{n}$ wpada do najmniej prawdopodobnego przedziału w partycji $\mathcal{P}^{asin}$ w prawie $0.01m$ przypadkach częściej niż dla dobrego generatora. Wystarcza to by wartość statystyki (\ref{eq:chi_asin}) bardzo urosła. Tymczasem charakterystyka $\Slil{n}$ przyjmuje dla ciągu $10(0110)^*01$ wartość zero, a tym samym wpada do najbardziej prawdopodobnego przedziału. Dlatego testowi $\chi^2$ trudniej jest to wykryć.
%F
%Gdybyśmy jednak w powyższym eksperymencie wykorzystali $m = 100000$ ciągów, to również test iterowanego logarytmu zauważyłby zbyt duże odstępstwo. Wypływa stąd wniosek, że w celu wykrywania tego rodzaju wad generatorów lepiej postawić na liczbę ciągów, a nie na ich długość.
\subsubsection{Results of \texttt{TestU01} for \textsl{Flawed}}

We have run several general-purpose tests against \textsl{Flawed} generator.
For \texttt{SmallCrush} all tests (15/15) were passed while for \texttt{Crush} 
one out of 
83 tests failed (passed 82/83)\footnote{\texttt{Crush} performs 96 tests but it 
occurred 
that the file containing $10000 \times 2^{26}$ is too small (the 
file's size was $83 886 080 000$ bytes) to complete the test.}.

Another series of tests was performed using approach which uses a binary file
and in the case when more bits are needed than the file has, bits are reused. 
In  Figure~\ref{listing:rabbit} results of \texttt{Rabbit} test are 
presented.\\

\begin{figure}
\begin{subfigure}[t]{.4\textwidth}
\begin{minipage}{.4\textwidth}
\vspace{-1cm}
{\small
\begin{verbatim}
========= Summary results of Rabbit =====

 Version:          TestU01 1.2.3
 File: FlawedDyckMT_len26.bin
 Number of bits:   671088640000
 Number of statistics:  40
 Total CPU time:   01:30:19.61
 The following tests gave p-values 
    outside [0.001, 0.9990]:
 (eps  means a value < 1.0e-300):
 (eps1 means a value < 1.0e-15):

       Test                      p-value
 ------------------------------------------
 11  HammingWeight                eps  
 18  AutoCor                    1 - eps1
 20  Run of bits                 3.5e-4
 20  Run of bits                1.3e-10
 ------------------------------------------
 All other tests were passed 
 
\end{verbatim}
}
% \vspace{5cm} \quad
\end{minipage}
\caption{Results of \texttt{Rabbit} battery of tests from \texttt{TestU01} for 
10000 sequences 
of length $2^{26}$ 
of PRNG \textsl{Flawed}.}\label{listing:rabbit}
\label{fig:rabbit}
\end{subfigure}
\begin{subfigure}[t]{.05\textwidth}
 \quad
\end{subfigure}
\begin{minipage}{.55\textwidth}
\begin{subfigure}[t]{.95\textwidth}
\scriptsize
\begin{verbatim}
-----------------------------------------------
   N =  1,  n = 10000,  r =  0,   s = 32,
   L0 = 67108864,   L1 = 67108864
-----------------------------------------------
Number of degrees of freedom          :  998
ChiSquare statistic                   : 2049.57
p-value of test                       : eps*****
\end{verbatim}
\caption{\textsl{Flawed} parameters are known. Weakness is 
detected.}\label{listing:jstat}
\end{subfigure}

\begin{subfigure}[t]{.95\textwidth}
\scriptsize
\begin{verbatim}

--------------------------------------------
   N = 10000,  n = 1024,  r =  0,   s = 32,
   L0 = 65536,   L1 = 65536
 --------------------------------------------
Number of degrees of freedom       : 1010000
Chi-square statistic               : 1.01e+6
p-value of test                    :    0.90
\end{verbatim}
\caption{Results for unknown parameters of 
\textsl{Flawed}}\label{listing:jstat1}
\end{subfigure}

\begin{subfigure}[t]{.95\textwidth}
\scriptsize
\begin{verbatim}

--------------------------------------------
   N = 10000,  n = 64,  r =  0,   s = 32,
   L0 = 1048576,   L1 = 1048576
--------------------------------------------
Number of degrees of freedom     : 50000
Chi-square statistic             : 50131.79
p-value of test                  :     0.34
\end{verbatim}
\caption{Results for unknown parameters of 
\textsl{Flawed}}\label{listing:jstat2}
\end{subfigure}

\end{minipage}
\caption{Listings of the selected outputs of tests for \textsl{Flawed} 
generator.}
\end{figure}




The results (see listings from 
Figures~\ref{listing:jstat},\ref{listing:jstat1},\ref{listing:jstat2}) suggest 
that without a knowledge of (potentially secret) 
parameter $N$ of the \textsl{Flawed} PRNG one may have problems with 
figuring out that the generator is
not a good one. If someone knows parameter $N$ (here $N = 26$) in 
\textsl{Flawed} RNG then the output of \textsl{Flawed} 
still looks good (compare Figure~\ref{listing:jstat1} and 
Figure~\ref{listing:jstat2}).

% Swalk\_RandomWalk1 (N = 10000,  n = 1024,  r =  0,   s = 32,   L0 = 65536,   L1 
% = 65536)
% 
% Swalk\_RandomWalk1 (N = 10000,  n = 64,  r =  0,   s = 32,   L0 = 1048576,   L1 
% = 1048576) (flawed64)
% 
% 
% \textcolor{red}{DOKONCZYC}
%  
% \subsubsection{NIST Test Suite}
% 
% For  $m=10000$ sequences of length 
% $n=2^{15}$, the ASIN test already returns $p$-value 0.000.
% For comparison, for this parameters we ran  
% we ran a battery NIST Test Suite. 
% Results are given in Table \ref{tab:flaw_nist}.
% For each sequence the corresponding $p$-value is was calculated. 
% NIST adopted two ways to interpret a set of $p$-values: a) examination of proportion of sequences that pass 
% a certain test; b) testing the uniformity of $p$-values (for truly random sequences they should be 
% uniformly distributed in $[0,1]$). 
% \par 
% Values in the columns C1,$\ldots,$ C10 represent number of $p$-values falling into intervals 
% $[0.0, 0.1), [0.1,0.2),\ldots,[0.9,1]$. Values in P-VALUE column represent the results for uniformity testing 
% of $p$-values, value in PROPORTION column represent proportion of sequences that pass a given test.
% The character $*$ denotes that the PRNG failed given test (more exactly: given interpretation of a set of $p$-values).
% For detailed description of results' interpretation see \cite{Rukhin2010}.
% Note that some tests from NIST Test Suite detected the flaw, but most did not.
% 
% \begin{table*}[t!]
% \scriptsize
% \centering
%  \caption{Partial results from the \texttt{finalAnalysisReport.txt} file produced by NIST Test Suite 
%  applied for $10^4$ sequences of length $2^{15}$ of flawed generator.}\label{tab:flaw_nist}.
%  \begin{tabular} {|p{0.5cm}|p{0.5cm}|c|c|c|c|c|c|c|c|l|l|c|c|c|c|c|c|c|c|}   
%  \hline 
% % ------------------------------------------------------------------------------                                                                                                       
% %  C1  C2  C3  C4  C5  C6  C7  C8  C9 C10  P-VALUE  PROPORTION  STATISTICAL TEST       
% 
% % ------------------------------------------------------------------------------                                                                                                       
% % 987 1036 980 961 1099 798 925 981 993 1240  0.000000 * 9896/10000    Frequency                                                                                                       
% % 990 1013 949 981 1013 1011 996 987 1007 1053  0.682410   9898/10000    BlockFrequency                                                                                                
% % 985 964 894 1120 889 832 1084 902 1117 1213  0.000000 * 9889/10000    CumulativeSums                                                                                                 
% % 1010 996 857 1100 868 829 1158 875 1051 1256  0.000000 * 9892/10000    CumulativeSums                                                                                                
% % 947 998 948 921 1001 1009 974 1079 1065 1058  0.001793   9910/10000    Runs                                                                                                          
% % 1119 992 1026 964 936 1081 1002 925 987 968  0.000102   9794/10000 *  LongestRun                                                                                                     
% % 1502   0 2865   0   0   0 5633   0   0   0  0.000000 * 10000/10000 *  Rank                                                                                                           
% % 1040 1111 518 1366 1753   0 2015   0 1107 1090  0.000000 * 9791/10000 *  FFT  
% C1& C2 & C3 & C4 & C5 & C6 & C7 & C8 & C9 & C10 &  \tiny P-VALUE & \tiny PROPORTION & \tiny STATISTICAL TEST       \\\hline
% % 987& 1036 & 980 & 961 & 1099 & 798 & 925 & 981 & 993 & 1240 & 0.000000  * & 9896/10000 &  Frequency \\
% % 990& 1013 & 949 & 981 & 1013 & 1011 & 996 & 987 & 1007 & 1053 & 0.682410 & 9898/10000 & BlockFrequency \\
% % 985& 964 & 894 & 1120 & 889 & 832 & 1084 & 902 & 1117 & 1213 & 0.000000  * & 9889/10000 & CumulativeSums \\ 
% % 1010& 996 & 857 & 1100 & 868 & 829 & 1158 & 875 & 1051 & 1256 & 0.000000  * & 9892/10000 & CumulativeSums \\
% % 947& 998 & 948 & 921 & 1001 & 1009 & 974 & 1079 & 1065 & 1058 & 0.001793 & 9910/10000 & Runs  \\
% % 1119& 992 & 1026 & 964 & 936 & 1081 & 1002 & 925 & 987 & 968 & 0.000102 &  9794/10000  * & LongestRun \\
% % 1502& 0 & 2865 & 0 & 0 & 0 & 5633 & 0 & 0 & 0 & 0.000000  * & 10000/10000 * & Rank  \\
% % 1040& 1111 & 518 & 1366 & 1753 & 0 & 2015 & 0 & 1107 & 1090 & 0.000000  * & 9791/10000  * & FFT \\\hline
% 
% 976 & 1043 & 972 & 1007 & 943 & 1053 & 1029 & 960 & 924 & 1093 & 0.001907 & 9907/10000 & Frequency \\
% 1015 & 999 & 927 & 972 & 1015 & 971 & 991 & 983 & 1029 & 1098 & 0.032705 & 9905/10000 & BlockFrequency \\
% 956 & 982 & 1066 & 996 & 928 & 1028 & 1005 & 996 & 956 & 1087 & 0.008428 & 9901/10000 & CumulativeSums \\
% 987 & 1027 & 951 & 967 & 1052 & 950 & 1011 & 977 & 938 & 1140 & 0.000101 & 9918/10000 & CumulativeSums\\ 
% 1042 & 930 & 972 & 1008 & 997 & 986 & 993 & 995 & 957 & 1120 & 0.004239 & 9886/10000 & Runs \\
% 1013 & 1015 & 1037 & 1014 & 1001 & 1008 & 947 & 988 & 989 & 988 & 0.812723 & 9809/10000  * & LongestRun \\
% 1006 & 869 & 1136 & 1016 & 1262 & 671 & 1466 & 864 & 778 & 932 & 0.000000  * & 9803/10000  * & Rank \\
% 1146 & 928 & 987 & 1055 & 868 & 995 & 1076 & 949 & 993 & 1003 & 0.000000  * & 9778/10000  * & FFT \\
% 1078 & 939 & 1008 & 999 & 1048 & 1027 & 978 & 1006 & 976 & 941 & 0.041709 & 9787/10000  * & OverlappingTemplate\\
% %10000 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0.000000 * &   0/10000  * & Universal\\
% 2017 & 1305 & 1154 & 1083 & 969 & 911 & 755 & 700 & 596 & 510 & 0.000000  * & 9576/10000  * & ApproximateEntropy\\
%  5 & 9 & 2 & 6 & 6 & 3 & 5 & 4 & 6 & 8 & 0.494392 & 53/54 & RandomExcursions\\
%  6 & 4 & 5 & 4 & 6 & 5 & 7 & 4 & 6 & 7 & 0.971699 & 54/54 & RandomExcursions\\
%  9 & 5 & 2 & 1 & 5 & 6 & 4 & 8 & 4 & 10 & 0.075719 & 54/54 & RandomExcursions\\
% 11 & 4 & 7 & 3 & 6 & 6 & 2 & 5 & 9 & 1 & 0.040108 & 51/54 & RandomExcursionsVariant\\
%  10 & 6 & 5 & 3 & 5 & 5 & 2 & 7 & 6 & 5 & 0.455937 & 53/54 & RandomExcursionsVariant\\
%  8 & 9 & 4 & 1 & 6 & 6 & 7 & 4 & 5 & 4 & 0.350485 & 53/54 & RandomExcursionsVariant\\
%  9 & 8 & 3 & 1 & 10 & 9 & 4 & 2 & 6 & 2 & 0.011791 & 53/54 & RandomExcursionsVariant\\
% 1201 & 935 & 1038 & 983 & 1005 & 949 & 971 & 951 & 978 & 989 & 0.000000  * & 9682/10000  * & Serial\\
% 1214 & 980 & 1037 & 1013 & 886 & 1001 & 934 & 925 & 1025 & 985 & 0.000000  * & 9697/10000  * & Serial\\
% 1112 & 875 & 931 & 933 & 1038 & 1057 & 1057 & 1073 & 966 & 958 & 0.000000  * & 9731/10000  * & LinearComplexity\\\hline 
% \end{tabular}
% \begin{flushleft}
%  
% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
% \par \noindent
% \texttt{The minimum pass rate for each statistical test with the exception of the
% random excursion (variant) test is approximately = 9870 for a
% sample size = 10000 binary sequences.
% }
% \medskip\par \noindent
% \par\texttt{The minimum pass rate for the random excursion (variant) test
% is approximately = 51 for a sample size = 54 binary sequences.} \par
% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
% 
% \end{flushleft}
% 
% \end{table*}


==> sections/fflawed.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Hypothetical flawed PRNG %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \textcolor{red}{UWAGA: juz w Section 1 nie ma ``inherent limitations'' z NISTa...``}
% Describing NIST SP800-22 Test Suite in Section  \ref{sec:intro} we pointed out 
% some of its inherent limitations
% directly related to the approach applied for statistical testing. Namely, this 
% test suite focuses only on the quality
% of a single binary sequence produced by a PRNG and does not take into account 
% the set of all bit strings
% as a whole. 


In this section we present $\textsf{Flawed}_{rng, N, \tau}$ -- a family of PRNGs . The family depends on three parameters: $rng$ -- is a PRNG (\eg MersenneTwister), $N$ is a small integer parameter (\eg $N = 30$) and $\tau \in [0, 1]$. $\textsf{Flawed}_{rng, N, \tau}(seed)$  generates the same output as $rng(seed)$ for
a fraction $1-\tau$ of all possible seeds. For the remaining fraction   $\tau$ of seeds \textsf{Flawed} outputs bits such that the corresponding walk of the length $2^N$ spends exactly half  of the time ($2^{N-1}$ steps) above zero and exactly half the time below zero.

% Let us consider some hypothetical PRNG which usually generates 
% sequences which ``look'' random, but 
% with some non-negligible probability (\eg for some subset of seeds) its output 
% is biased and far from truly random.
% % Such a flawed sequence will be surely recognized by NIST Test Suite as 
% % non-random, but this deviation probably will not cause
% % considering whole PRNG as ``not good''. However, its output will be easily 
% %distinguishable from uniform bit strings.
% This issue was carefully discussed in Section 3 of \cite{Wang2015}, where some 
% specific examples of such PRNGs were presented.
% 
% The following example gives an insight on how this kind of weaknesses in 
% generator's output may be detected by the ASIN test.
% \par 
% Before introducing the PRNG we need to define \textsl{Dyck paths} and say how to 
% simulate one randomly.

\subsection{Dyck Paths}
To generate walks with the aforementioned property we will use Dyck paths --  walks starting and ending at 0 with a property 
that for each prefix the number of ones is not smaller than the number of zeros.

% \smallskip\par 
% \pl{PL: dopisalem, ze startuja i koncza w zerze.}

% \smallskip\par 
% \pl{PL: ponizej $n$ i $\mathfrak{n}$, ktore jednak oznaczaly dlugosc ciagu... w tym rozdz. jest to $2^N$..
% Moze tak: pozmieniac w dyck pathach  $n$ i $\mathfrak{n}$ na cos innego, a gdzies napisac, ze $N=\log_2 n$ ?}



\begin{deff}
 A sequence of $n = 2\mathfrak{n}$  bits $B_1,\ldots, B_{2\mathfrak{n}}$ is called a \textsl{Dyck path} if
 the corresponding walk $S_k$ fulfills: $S_k=\sum_{i=1}^k(2B_i-1)\geq 0, 
k=1,\ldots,2\mathfrak{n}-1$ and $S_{2\mathfrak{n}}=0$.
 A set of all Dyck paths of length $2\mathfrak{n}$ is denoted by $\mathcal{D}_{2\mathfrak{n}}$.
\end{deff}
Thus, a Dyck path of length $2\mathfrak{n}$ corresponds to a valid grouping of $\mathfrak{n}$ pairs of 
parentheses,
we have $|\mathcal{D}_{2\mathfrak{n}}|=C_\mathfrak{n}={1\over \mathfrak{n}+1}{2\mathfrak{n}\choose \mathfrak{n}}$ (the $\mathfrak{n}$-th Catalan number).



\subsection{Sampling Dyck Paths}
We are interested in generating Dyck paths uniformly at random. To achieve this goal
we use the following three ingredients.

\paragraph{(1) Walk sampling}
Let $\mathcal{I}_{2\mathfrak{n}+1}^{-1}$ be the set of 
sequences of bits $B_1,\ldots, B_{2\mathfrak{n}+1}$ such that the corresponding walk
$S_k$ ends at $-1$, \ie $S_{2\mathfrak{n}+1}=-1$. 
One can simulate uniformly at random  $I\in\mathcal{I}_{2\mathfrak{n}+1}$: it is enough to
make a random permutation of the vector of bits $(0,\ldots,0,1,\ldots,1)$,
where there are $\mathfrak{n}+1$ zeros and $\mathfrak{n}$ ones. 

\paragraph{(2) $f_{\textsf{Dyck}}$ transformation}
One can obtain a Dyck path of length $2\mathfrak{n}$ from $I\in\mathcal{I}_{2\mathfrak{n}+1}^{-1}$ via Algorithm~\ref{alg:fdyck}.
\begin{algorithm}[H]
\caption{$f_{\textsf{Dyck}}(I)$}\label{alg:fdyck}
\hspace*{\algorithmicindent} \textbf{Input}: $I=(B_1,\ldots,B_{2\mathfrak{n}+1})\in \mathcal{I}_{2\mathfrak{n}+1}^{-1}$ \\
\hspace*{\algorithmicindent} \textbf{Output}: corresponding Dyck path $f_{\textsf{Dyck}}(I)$
\begin{algorithmic}[1]
% \Procedure{asd}{asd}
\State $S_k = \sum_{i=1}^k(2B_i-1)$ for $k = 1, \ldots, 2\mathfrak{n}+1$
\State $s=\textrm{argmin}\{ S_k : k \in \{1, \ldots, 2\mathfrak{n}+1\}\}$
\State $f_{\textsf{Dyck}}(I) = (B_{s+1}, \ldots, B_{2\mathfrak{n}+1}, B_1, \ldots, B_{s-1})$\\
\Return $f_{\textsf{Dyck}}(I)$
\end{algorithmic}
% \caption{asd}
\end{algorithm}
\noindent
$f_{\textsf{Dyck}}$ transforms $I\in\mathcal{I}_{2\mathfrak{n}+1}^{-1}$ into a Dyck path because:
\begin{enumerate}
 \item $I$ has exactly $\mathfrak{n}+1$ zeros and $\mathfrak{n}$ ones.
 \item since $s = \textrm{argmin}\{ S_k : k \in \{1, \ldots, 2\mathfrak{n}+1\}\}$ then $B_s = 0$ and after $B_s$ is removed then $f_{\textsf{Dyck}}(I)$ has exactly $\mathfrak{n}$ bits equal $0$ and $\mathfrak{n}$ bits equal $1$; and 
 \item from the definition of $s$  (which enforces in particular that $B_s = 1$), the walk that corresponds to bits $(B_{s+1}, \ldots, B_{2\mathfrak{n} + 1}, B_1, \ldots, B_{s-1})$ cannot go below $0$.
 \end{enumerate}


An example of the $f_{\textsf{Dyck}}$ transformation is presented on the Figure~\ref{fig:p_dyck}.

\input{figures/flawed}

\paragraph{(3) Cycle lemma} The correspondence between the set $\mathcal{I}_{2\mathfrak{n}+1}^{-1}$ and the set $\mathcal{D}_{2\mathfrak{n}}$ is expressed 
by the  {Cycle Lemma}~\cite{Dvoretzky47}.

\begin{lem}[Cycle Lemma]\label{lem:cycle}
 For any $I\in \mathcal{I}_{2\mathfrak{n}+1}^{-1}$ the path $f_{\textsf{Dyck}}(I)$ is a Dyck path.
 Moreover, any Dyck path in $\mathcal{D}_{2\mathfrak{n}}$ is the image of exactly $2\mathfrak{n}+1$ 
paths in
 $\mathcal{I}_{2\mathfrak{n}+1}^{-1}$.
\end{lem}

\noindent 
Thus,  to obtain a  \textsl{random sampling of a Dyck path} of length $2\mathfrak{n}$ one needs to:

\begin{algorithm}[H]
\caption{$\textsf{sampleDyckPath}(\mathfrak{n}, rng, seed)$}\label{alg:sample_dyck}
\hspace*{\algorithmicindent} \textbf{Input}: $\mathfrak{n}$ -- integer\\ \hspace*{\algorithmicindent} \qquad \qquad $rng$ -- pseudorandom generator\\
\hspace*{\algorithmicindent} \qquad \qquad $seed$ -- seed\\
\hspace*{\algorithmicindent} \textbf{Output}: $P$ -- sampled Dyck path of the length $2 \mathfrak{n}$ 
\begin{algorithmic}[1]
% \Procedure{asd}{asd}
 \State $x = (B_1, \ldots, B_{2\mathfrak{n}+1})$  where $B_1 = \ldots = B_{\mathfrak{n}+1}=0$ and $B_{\mathfrak{n}+2} = \ldots = B_{2\mathfrak{n}+1}=1$
 \State use bits of $rng(seed)$ to generate a permutation $\pi$ of $2\mathfrak{n}+1$ elements 
 \State $I = (B_{\pi(1)}, \ldots, B_{\pi(2\mathfrak{n}+1)})$
 \State $P = f_{\textsf{Dyck}}(I)$\\
 \Return $P$
\end{algorithmic}
% \caption{asd}
\end{algorithm}

\pl{PL: \textsf{sampleDyckPath} nie jest nigdzie nizej uzyte..}


% 
% 
% \medskip\par 
% Now we are ready to present our \textsl{Flawed} PRNG. It takes as an input:
% \begin{itemize}
%  \item \textsl{rng} -- another PRNG (\eg Mersenne Twister MT19937-64),
%  \item $N$ -- the maximal number of bits returned by the generator is limited 
% by 
% $2^N$,
%  \item $\tau$ -- parameter which decides how often the output is modified,
%  \item \textsl{seed} -- the seed. 
% \end{itemize}

\subsection{\textsf{Flawed} generator}
As we mentioned at the beginning of this section, the $\textsf{Flawed}_{rng, N, \tau}(seed)$ generators work exactly as the underlying generator 
for a fraction $(1-\tau)$ of  seeds (lines 1-2 of the Algorithm~\ref{alg:flawed}). For the  the remaining fraction   $\tau$  of  seeds (line (3) ``else'' branch) output is generated in the following way.
\begin{enumerate}
 \item The first $2^{N-2}$ bits are exactly the same as the first bits of $rng(seed)$ (line 4).
 \item To generate next $2^{N-2}$ bits, a pseudorandom permutation $\pi$ is generated and output bits are a negations of the corresponding (via $\pi$) bits (lines 5-8). 
 As a result, there is the same number of zeros and ones in first  $2^{N-1}$ bits (\ie the corresponding walk is at zero at step $2^{N-1}$).
 
 \item The remaining $2^{N-1}$ of the block are obtained in such a way that the whole block of $2^N$ output bits has the property that the corresponding walk spends the same number of steps above and below 0 (line 9).
\end{enumerate}


\begin{algorithm}[H]
\caption{$\textsf{Flawed}_{rng, N, \tau}(seed)$}\label{alg:flawed}
\begin{algorithmic}[1]
% \Procedure{asd}{asd}
\If{$seed \neq 0 \bmod \lceil 1/\tau \rceil$} \\
  \quad \Return $rng(seed)$
\Else 
  \State $z_1 \ldots z_{2^{N-2}} \leftarrow rng(seed)$
  \State $\pi \leftarrow \textsf{RandPerm}(2^{N-2}, rng(seed))$
  \For{$i = 1$ to $2^{N-2}$}
    \State $z_{2^{N-2} + i} := 1 - z_{\pi(i)}$
  \EndFor
  \State $z_{2^{N-1}+1} \ldots z_{2^N} \leftarrow \textsf{DyckPaths}(N, z_1 
\ldots z_{2^{N-1}}, rng(seed))$ \\
  \Return $z_1 \ldots z_{2^N}$
\EndIf
\end{algorithmic}
% \caption{asd}
\end{algorithm}


% \begin{algorithm}[H]
% \caption{$\textsf{DyckPaths}(n, r_1 \ldots r_2^{n-1}, rng)$}\label{alg:flawed}
% \begin{algorithmic}[1]
% % \caption{asd}
% \State $S_n=\sum_{i=1}^n (2r_i-1)$
% \State $D_k = \mathbbm{1}\left(S_k > 0 \vee S_{k-1}>0 \right)$
% \State $O_0:=[l^{O}_0,r^{O}_0]:=[0,0]$
% \State $U_0:=[l^{U}_0,r^{U}_0]:=[0,0]$
% \State $n_O=\min\{i: l^{O}_i=\emptyset\}-1, |O_i|=r^{O}_i-l^{O}_i+1.$
% 
% \For{$i=1$ to $2^{n-1}$}
% \State $l^{O}_i=\min\{l^{O}_{i-1}< k\leq 2^{n-1}: D_k=1 \}$
% \State $r^{O}_i=\max\{l^{O}_i<k\leq 2^{n-1}: D_k=1\}$
% \State $O_i=\{l^{O}_i,\ldots,r^{O}_i\},$
% \State $U_i=\{l^{U}_i,\ldots,r^{U}_i\}, $
% \State $l_i=\min\{l^{U}_{i-1}< k\leq 2^{n-1}: D_k=0 \}$
% \State $r_i=\max\{l^{U}_i<k\leq 2^{n-1}: D_k=0\}$
% \State $n_U=\min\{i: l^{U}_i=\emptyset\}-1$
% \State $|U_i|=r^{U}_i-l^{U}_i+1.$
% \EndFor
% \end{algorithmic}
% \end{algorithm}
% 


%\textcolor{red}{PL: nie chcielismy tutaj od razu napisac, ze de facto to tylko arcus sinus tes wykrywa?}
% \begin{itemize}
Let us assume that lines 1--8 of Alg. \ref{alg:flawed} generated $\mathbf{z}_L=z_1 \ldots z_{2^{N-1}}$, the 
corresponding random walk spent $T_U(\mathbf{z}_L)$ time under 
 the $x$-axis and $T_O(\mathbf{z}_L)$ time
 over the $x$-axis ($T_U(\mathbf{z}_L) = 2^{N-1} - T_O(\mathbf{z}_L)$).
 The goal of the procedure $z_{2^{N-1}+1} \ldots z_{2^{N}} 
\leftarrow \textsf{DyckPaths}(N, z_1 \ldots z_{2^{N-1}}, rng)$ is to produce 
bits $\mathbf{z}_R = z_{2^{N-1}+1} \ldots z_{2^{N}}$ for which $T_U(\mathbf{z}_R) = T_O(\mathbf{z}_L)$ and 
$T_O(\mathbf{z}_R) = T_U(\mathbf{z}_L)$. Then if one concatenates sequences $\mathbf{z}_L$ and $\mathbf{z}_R$, for the 
corresponding random walk it holds that $T_U(\mathbf{z}_L\mathbf{z}_R) = T_O(\mathbf{z}_L\mathbf{z}_R)$.

The following is an informal description of the procedure 
$\textsf{DyckPaths}(N, z_1 \ldots z_{2^{N-1}}, rng)$:
	\begin{enumerate}
	  
% 	  \item[$\diamond$]
% 	  \item Denote the current half of the output as 
% $\mathbf{r}=(r_1,\ldots,r_{2^{n-1}})$,

	  \item The   walk  corresponding to $\mathbf{z}_L$ is given by $S_k=\sum_{i=1}^k (2z_i-1), k=1,\ldots,2^{N-1}$. 
Recall (\ref{eq:dk}): $D_k = \mathbbm{1}\left(S_k > 0 \vee S_{k-1}>0 \right)$.
	  
	  
	
	  
	  
% 	  \item[$\diamond$] 
\item Define $O_0:=[l^{O}_0,r^{O}_0]:=[0,0]$ and 
$O_i=\{l^{O}_i,\ldots,r^{O}_i\}, $ where 
	  $l^{O}_i=\min\{l^{O}_{i-1}< k\leq 2^{N-1}: D_k=1 \}, r^{O}_i=\max\{l^{O}_i<k\leq 2^{N-1}: D_k=1\}$, $n_O=\min\{i: l^{O}_i=\emptyset\}-1,
	   |O_i|=r^{O}_i-l^{O}_i+1.$
	  
% 	  \item[$\diamond$] 
\item Similarly, $U_0:=[l^{U}_0,r^{U}_0]:=[0,0]$ and 
$U_i=\{l^{U}_i,\ldots,r^{U}_i\}, $
	  where $l_i=\min\{l^{U}_{i-1}< k\leq 2^{N-1}: D_k=0 \}, r_i=\max\{l^{U}_i<k\leq 2^{N-1}: D_k=0\}$, $n_U=\min\{i: l^{U}_i=\emptyset\}-1, |U_i|=r^{U}_i-l^{U}_i+1.$
	  
	  \medskip\par 
	  $O_i$ and $U_i$ are the intervals for which random walk is over $x$-axis and 
	  under $x$-axis respectively\footnote{For example, if $(D_1,\ldots,D_{16})=(1,1,0,0,1,1,1,1,0,0,0,0,0,0,1,1),$
	  then  $O_1=[1,2], O_2=[5,8], O_3=[15,16], U_1=[3,4], U_2=[9,15]$.}.
	  
	 
	  
	  
% 	  \item[$\diamond$] 
\item In the second half, the bits will be chosen 
	  so that the walk will be $\sum_i |O_i|$ steps \textsl{under} $x$-axis 
	  and $\sum_i |U_i|$ over this axis. Dyck paths $DP_{U, i}$ of respective lengths $|U_1|, \ldots, |U_{n_U}|$ and reflected (simply replacing bits $0\leftrightarrow 1$) Dyck paths 
	  $DP_{O, i}$ of lengths $|O_1|,\ldots,|O_{n_O}|$ are generated: $DP_{U, i} = \textsf{sampleDyckPath}(|U_i|/2, rng, h(seed, U, i))$, $DP_{O, i} = \textsf{sampleDyckPath}(|O_i|/2, rng, h(seed, O, i))$ 
	  (for some hash function $h$).
\item Relative ordering of the paths (generated in the previous step) is obtained from a permutation $\pi \leftarrow  \textsf{RandPerm}(n_O + n_U, rng(seed))$
	  of $n_O+n_U$ numbers.
	  
	  \item Return computed bits.
	   
	\end{enumerate}
% 	
% 	
% 	sequence described by the regular expression 10(0110)*01,
% 	      \ie binary string starting with 10, followed by repeated runs of 0110 and ending with 01. 
% 	
% \end{itemize}

% \pl{ponizsze do zmiany.. - amoze tutaj wywalic info z $N$ i $\tau$? tylko juz w experimental results dac}
Ten  sample trajectories of \textsf{Flawed} (all from \textsl{Dyck path}-based part 
of   Algorithm \ref{alg:flawed}) are given in Figure~\ref{fig:flaw} (where $\textsf{Flawed}_{rng, N, \tau}$ is taken for
the following parameters: $N = 2^{26}$, \textsl{rng} -- MersenneTwister and 
 $\tau = 1/100$).
\begin{figure}[H]
\centering
%[width=\columnwidth]
%\includegraphics[scale=0.5]{figures2/flaw}
\includegraphics[scale=0.16]{figures/flawed.png}

\caption{10 trajectories of length $2^{18}$ of \textsl{Flawed} generator for seeds such that $seed = 0\bmod \lceil{1/\tau}\rceil$.}\label{fig:flaw}
\end{figure}


==> sections/intro_old.tex <==
% tutaj a'la Wang Nicole \cite{Wang2015}, np. o p-value... i moze troche o ich rozdziale
% \par 
% ``3. Limitations of  NIST SP800-22''
% \textcolor{red}{Tu chyba pasuje czesc / (calosc?) rozdzialu 2.3}
%\subsection{Testing PRNGs}
%\textcolor{red}{Przeniesione... wczesniej to bylo w pod koniec rozdz. 2., ale calosc prawie pasuje jako wstep.}  
%\textcolor{red}{Moze to przeniesc (choc w czesci) do wstepu? Chyba tam by bardziej pasowalo.}  
Random numbers are key ingredients in various applications, e.g., in cryptography (e.g., 
for generating a secret/public key) or
in simulations (e.g., in Monte Carlo methods), just to mention a few. No algorithm can produce truly random numbers.
Pseudo random number generators (PRNGs) are used instead. These are deterministic algorithms which produce 
numbers which we expect to resemble truly random ones \textsl{in some sense}.
In order to evaluate whether a given PRNG is sound and can be applied for purposes where strong
pseudorandomness is required, various tests are applied to its output. The main goal of these tests is to check if the sequence of numbers 
$\mathbf{U} = (U_1, U_2, \ldots, U_n)$ (or bits, depending on the actual implementation) produced by PRNG
resembles a sequence of elements generated independently and uniformly at random.
Due to popularity and significance of the problem, a variety of testing procedures have been developed in recent years.
Such statistical tests are generally aimed at detecting various deviations in generated sequences what allows for
revealing flawed PRNG implementations producing predictable output.
These techniques can be divided into several groups according to the approach used for verifying the quality of generators.

The first class of procedures encompasses classical tools from statistics like Kolmogorov-Smirnov test or 
Pearson's chi-squared test which are used for comparing  theoretical and empirical distributions of appropriate
statistics calculated for PRNG's output. %  by determining the p-value and comparing it with chosen significance level. 
It is also possible to adapt tests of normality like Anderson-Darling or Shapiro-Wilk tests for appropriately transformed
pseudorandom sequences.
% However, this kind of methods tests only whether the output of a PRNG is distributed uniformly.
% Nevertheless, it is also possible in theory to extend them for veryfing indepencence by taking $t$-tuples
% of the outputted sequence and verifying whether they are uniformly distributed in $t$-dimensional hypercube, but
% this approach is of little use.

Another category of testing methods relies on the properties of sequences of independent and identically distributed
random variables. Based on the original sequence $\mathbf{U}$ returned by the examined PRNG we are able to obtain
realizations of other random variables with known theoretical distributions. Some examples of probabilistic laws
used in practice in this kind of tests can be found e.g., in \cite{Knuth2}. They include such procedures like gap
test, permutation test and coupon collector's test, just to name a few (see \cite{Knuth2} for more detailed treatment).
These methods have also the advantage that they implicitly test independence of generator's output.

The main issue with such methods is that a single statistical test looks only at some specific property that holds for
sequences of truly random numbers. If a PRNG passes given test, it only implies that generated sequences have this
particular property. Hence, for practical purposes bundles of diverse tests are created.
Such a test bundle  consists
of a series of individual procedures based on various stochastic laws from probability theory.
A PRNG is then considered as good if the pseudorandom sequences it produces pass all tests in a given bundle.
Some examples of such test suites are Marsaglia's Diehard Battery of Tests of Randomness from 1995, 
Dieharder developed by Brown et al. (cf. \cite{Dieharder}), TestU01 implemented by L'Ecuyer and Simard
(see \cite{TestU01,TestU01_guide}) and NIST Test Suite \cite{NISTtests}.
The last one, designed by National Institute of Standard and Technology is currently
considered as one of the state-of the art test bundles and thus widely used for practical purposes. For that reason we shall
briefly summarize its most important features. Comprehensive description of all its testing procedures together with additional 
technical and implementation details can be found in \cite{Rukhin2010}.
NIST Test Suite SP800-22 \cite{NISTtests} comprises of 15 specific tests for determining whether pseudorandom 
sequences passed as the input can be treated as good. NIST SP800-22 includes such methods like monobit test for checking
what  the proportion of zeros and ones in tested sequence is, runs test taking into account the lengths of subsequences
consisting of runs of identical bits and serial test for checking for given $k$ what the frequencies of occurrences
of all $k$-bit  overlapping patterns are. The procedures in NITS SP800-22 proceed as follows.
In each case the null hypothesis is that the tested sequence is a 
realization of truly random bit sequence. For each test $m$ sequences are generated using tested PRNG. Then for each sequence
the test is carried out with selected significance level $\alpha$ (by default $\alpha = 0.01$) resulting in outputting the 
corresponding $p$-value. The tested sequence is considered to be random if $p \geq \alpha$. A PRNG is then accepted as 
sound if the fraction of all input sequences passing the test is about $1-\alpha$. The results can be further inspected by e.g.,
analyzing the distribution of obtained $p$-values, as suggested by NIST (cf. \cite{Rukhin2010, NIST2014}).

Although this approach seems to be reliable, it has, however, some inherent limitations. Namely, the key issue is that NIST tests 
focus merely on characteristics of single binary strings returned by tested PRNG rather that treating them as a whole.
This problem can be explained by   the following example. Suppose that we have some 
generator $G_1$ which is considered as good by the NIST Test Suite and let us consider another PRNG, $G_2$ such that every 
hundredth sequence it produces will be some fixed or highly biased bit string (e.g., with number of 1s highly exceeding number of 0s), 
and in all the remaining cases it returns the output of $G_1$. $G_2$ will be likely recognized by NIST SP800-22 as strong PRNG
despite its obvious flaws (its output is easily distinguishable from that of truly random generator). This drawback are
formalized and carefully discussed by Wang and Nicol  \cite{Wang2015} in Section 3. They also reported that some PRNGs used
in practice, which are known to be weak, like Debian Linux (CVE-2008-0166) PRNG based on OpenSSL 0.9.8c-1 or standard C linear
congruential generator, pass the tests from NIST SP800-22 using testing parameters recommended by NIST. As we shall see, the 
method we propose is capable of detecting such flawed generators.


%\textcolor{red}{Czy wspomniec o spectral test i kolmogorov complexity? (jak tak, to odkomentowac w gens.tex)}
% Another method for evaluating PRNGs is so called spectral test proposed by Knuth in \cite{Knuth2}.
% It is mainly based on inspecting the distribution of successive blocks of pseudorandomrandom numbers produced by the generator
% treated as points in $t$-dimensional space. For some LCG and MCG one can observe e.g. that such points mainly lie on very 
% limited % number of (t-1)-dimensional hyperplanes, what is uncommon for sequence of truly random numbers.
%
% There are also methods of testing PRNG that make use of some other measures defined for binary string like Kolmogorov complexiy
% (for the definition and applications of Kolmogorov complexity see e.g. \cite{Li2008}).

A very interesting approach for testing PRNGs was presented in \cite{Kim2008}. The concept of their tests is based on the
properties of random walk on $\mathbb{Z}_n$ with 0  being an absorbing state (also known as gambler ruin problem), more 
 precisely, on the time till absorption.
The authors    propose three different variants of the test. The general idea of the basic procedure 
is the following. For fixed $p \in (0,1)$ and $x \in \mathbb{Z}_n$, the output $\mathbf{U} = (U_i)$ of a PRNG is treated as 
numbers from unit interval and used to define a random walk starting in $x$ such that if $U_i < p$ and the process is in state $s$,
then it moves to $(s+1) \mod n$, otherwise to $(s-1) \mod n$. The aim of this test is to compare theoretical and empirical 
distributions of time to absorption in 0 when starting in $x$. Based on the values of testing statistics, the PRNG is then either 
accepted or rejected.  The authors reported some ``hidden defects'' in the widely used Mersenne Twister 
generator. However, one has to be very careful dealing with randomness: it seems like re-seeding PRNG with a fixed seed was 
an error which led to wrong conclusions. The  criticism was raised by  Ekkehard and Grønvik \cite{Ekke10},
authors also show that tests of Kim et al. \cite{Kim2008} performed \textsl{properly} do not reveal any defects in Mersenne Twister PRNG.
Recently, authors in \cite{Lorek2017a} proposed another gambler ruin based procedure for testing PRNGs.
Authors exploited formulas for winning probabilities for arbitrary  sequences $p(i), q(i)$, (\ie  winning and losing probabilities 
depend on the current fortune) which are the parameters  of the algorithm.


In recent years a novel kind of testing techniques has been introduced for more careful verification of generators.
The core idea of this class of methods is based on  observation that the binary sequence $(B_i)$ produced by a PRNG,
after being properly rescaled, can be interpreted as a one-dimensional random walk $(S_i)_{i \in \mathbb{N}}$ with 
$S_n = \sum_{i=1}^{n} X_i$, where $X_i = 2 B_i - 1$. For random walks defined by truly random binary sequences a wide range of 
statistics has been considered over the years and a variety of corresponding stochastic laws has been derived
(see e.g. \cite{Feller1968}) . For a good PRNG we may expect that its output behaves as $S_n$. Hence, the following idea comes to
mind: choose some probabilistic  law that holds for truly random bit sequences and compare the theoretical distribution of the 
corresponding statistics with the empirical distribution calculated for $m$ sequences produced by examined PRNG in $m$ 
independent experiments. This comparison can be done e.g., by computing the $p$-value of the appropriate test statistics under the 
null hypothesis that the sequence generated by PRNG is truly random. Another concept named \emph{statistical distance based
testing} was suggested in \cite{Wang2015}, which relies on calculating statistical distances like e.g., total variation or 
separation distance (cf. formulas (\ref{eq:dtv}) and (\ref{eq:sep}), respectively) between the  theoretical and the empirical distribution for 
considered characteristics and rejecting PRNG  if the distances are above some threshold.
Such approach was adopted in \cite{Wang2015}, where the authors derive their test statistics from Law of Iterated Logarithm 
for random walks. The procedure we propose uses similar methodology and is based on Arcsine Law.  
In the following Section \ref{sec:rw} we will recall the aforementioned stochastic laws for random walks,
whereas the testing methods will be described in Section \ref{sec:arcsine_tester}.
%\paragraph{Notations used}
Through the paper we will denote by $[n]$ the set $\{1, \ldots, n\}$.


==> sections/intro_old_gambler.tex <==
% !TEX root = ../main_PRNG_gambler.tex


\section{Introduction}

Random numbers are a key ingredient of cryptography. No deterministic algorithm 
can generate truly random numbers. Pseudorandom number generators (PRNGs)  are the algorithms
outputting numbers which \textsl{should} be  indistinguishable, in some sense, from truly 
random numbers. Ones do better than the others. The aforementioned indistinguishability is defined in quite 
a general way, usually one says about the ability of  \textsl{some} adversary to  distinguish 
the output of PRNG from truly random numbers in \textsl{some} way. This leads to conclusion that we can never 
prove that some PRNG returns numbers which are indistinguishable from truly random ones.
All we can do is to invent some tests and state which PRNGs fail and which do not fail them. 
The better the PRNG the more tests should be passed. Most of the tests are based on some results from 
pobability theory. Many of them use some known facts from bin-and-boxes schemes. For example, $n$ consecutive bits from PRNG output can be treated as
an integer from $[0,\ldots, 2^n-1]$ and we can imitate some box-and-bins scheme \textcolor{red}{(wymienic kilka)}. If the numbers were \textsl{truly} random then 
we know something about some statistics (e.g., if we throw $N=2^n$ balls into $N$ bins then the 
maximum load is of order $\ln N/\ln\ln N$ w.h.p). Other class of tests are based on results concerning random walks, e.g.,
hitting-time distributions \cite{Kang2005}, duration of gambler's ruin game \cite{Kim2008}, law of iterated algorithm \cite{Wang2015}.
% ddgabmler's-like problems.
We can then compare the realization obtained from PRNG with 
what \textsl{should} happen. There are always  lots of issues: what $n$ should we choose? How many samples should we collect?, etc.
There are some famous collections  of tests, e.g., NIST800-90A Test Suite \cite{NIST2014}, DieHard tests (considered deprecated),
TestU01 tests \cite{TestU01}. The last one by L'Ecuyer and  Simard is considered state of the art in the field.
The newer and newer tests are being invented, as the area caught lots of attention recently.
There is a large number of publications introducing one test, which usually tests one or few aspects of PRNGs.
\marginpar{\tiny gdzies by sie przydaly, ze troche testow jest opartych o simple random walk... gamblery, LIL itp}
\par \medskip
\textbf{\todo{nazwa do zmiany} Be careful when dealing with randomness ...}
\par
However, one has to be \textsl{very} careful when dealing with randomness:
The tests of Kim et al. \cite{Kim2008} (titled ``Tests of randomness by the gambler’s ruin algorithm'') 
were based on expectation and variation of duration of gambler's game. Assume initially gambler has $s$ dollars 
and bank has $N-s$ dollars. At  each step he either wins a dollar with probability $p$ or loses a dollar with the remaining probability. 
The game ends when gambler is broke (reaches $0$) or he wins (reaching $N$). The expectation and variance 
of duration of the game is known in specific cases (authors' algorithms $A1-A5$ and $B1-B5$, for their algorithms $C1-C5$ it was not known earlier).
Authors split the output of  PRNG into intervals of some prespecified number of bits, each sequence is then treated 
as a binary representation of number from interval $[0,1]$. For starting point $s$ the PRNG is used until 0 or $N$ is reached,
whole procedure is reapeated 20000 times and sample mean of game's duration is calculated, finally standard $Z$-test is performed.
Authors do not rely on one starting point $s$, but for $N=300$ they start the gambler's game for each $s=1,\ldots,N$
and they \textsl{judge} the PRNG depending on for how many  starting points it fails. They claim 
``hidden defects'' in some generators, including commonly used Mersenne Twister generators \cite{Matsumoto1998}. \textsl{However}, 
for each starting point $s$  the same seed is used at each iteration. Thus, the games cannot be treated as indepnendent.
For example, this is one of obivous dependencies: if the game started at say $10$ finishes at 0 (i.e., losing), then so do games started at $1,\ldots,9$ (!).
This also translates in obvious way to game's duration. The authors were 
aware that ``the $Z$-values corresponding to different starting points are highly correlated'', nevertheless 
they proceeded with ``we can regard a $Z$-value to each starting point as a separate test result''.
The critisism was raised by  Ekkehard and Grønvik \cite{Ekke10}, where they baldly pointed out the mistakes. 
Moreover, Ekkehard and Grønvik \cite{Ekke10} show that tests of Kim et al. \cite{Kim2008} performed \textsl{properly}
do not show any defects in Mersenne Twister (and some other) PRNG.  
\par \medskip
\textbf{(TO DO:) Our approach}
\par
Most of random-walk-based tests (including tests from  \cite{Kim2008}) perform the following:
\begin{itemize}
 \item[S1] Split the sequence of bits returned by PRNG into sequences of pre-defined lenght (usually 16 or 32-bit length)
 \item[S2] Treat each one as an integer number or as number from $[0,1]$
 \item[S3] Perform some \textsl{walk} (e.g., go \textsl{left} or \textsl{right}) according to the number obtained in S2 
 \textsl{indepnendently} of current state.
 \item[S4] Iterate S1-S3, calculate some statistics and compare them to known facts about the statistic (distribution,
expectation etc). 
\end{itemize}

The main drawback of above procedures are steps S1 and S3. Imagine gambler's ruin problem where at each step 
we are either to go left or right with probability $1/2$. Then, treating consecutive 32 bits as binary notation of a number,
we actually test every 32-nd bit. Of course if we know that the probability is $1/2$ we can simply apply 1-bit long sequence. 
However, such test can overlook some dependencies between bits. We obviate the obstacle by applying as many bits as is needed
(see Section \ref{sec:BitTracker}  on  \texttt{BitTracker}) and by using varying probabilities (which depend on current state).
The latter feature also eliminates the drawback of S3. \par 
In spirit, our approach is similar to  Kim et al. \cite{Kim2008}, we also use gambler's ruin based test,
to be precise: it's generalized version. The details will be given in forthcoming sections. 
Let us here only state two points which differs our approach from \cite{Kim2008}.
\begin{itemize}
 \item[A1] We use varying probabilities of winning/losing, they depend on current fortune.
 \item[A2] We calculate/estimate winning probabilities instead of duration of the game.
\end{itemize}
The main reason for using winning probabilities instead of the duration of the game is because we are able 
to provide explicit formulas for these probabilities for generalized Gambler's ruin problem,
the game duration in such general case is an open problem.
%  
% 
% 
% \par 
% \cite{Kim2008b}  ``return time''
% \par 
% \cite{Kim2008} ``tests of randomness``
% \par 
% 
%   \cite{Ekke10} ''Re-seeding invalidates tests of random number generators``
%  \par 
%  \cite{Lorek2015b} ''Gen. Gambler's ruin problem: explicit formulas via duality``
%  \par 
%  
%  
 

==> sections/old.tex <==

\subsection{Conclustions table}
The observations are summarized in Table \ref{table:rw_laws}.
\begin{table*}
  \centering%
  \begin{tabular}{|l|l|l|l|l|}\hline
   & conv. in prob. & a.s. conv. & $\limsup$ a.s & $\liminf$ a.s \\[7pt]\hline
    LLN & ${S_n\over n}\stackrel{P}{\to}0$ & ${S_n\over n}\stackrel{a.s.}{\to}0$
    & $\displaystyle\limsup_{n\to\infty} {S_n\over n}=0$ & $\displaystyle\liminf_{n\to\infty}{S_n\over n}=0$ \\[7pt]\hline
    
    LIL & ${S_n\over 2n\log\log n}\stackrel{P}{\to}0$ & ${S_n\over 2n\log \log n}\stackrel{a.s.}{\nrightarrow }0$
    & $\displaystyle\limsup_{n\to\infty} {S_n\over 2n\log\log n}=1$ & $\displaystyle\liminf_{n\to\infty}{S_n\over 2n\log\log n}=-1$ \\[17pt]\hline
    
    
    CLT & $\forall x {S_n\over n}\stackrel{P}{\nrightarrow}x$ & $\forall x {S_n\over n}\stackrel{a.s.}{\nrightarrow }x$
    & $\displaystyle\limsup_{n\to\infty} {S_n \over n}=\infty$ & $\displaystyle\liminf_{n\to\infty}{S_n\over n}=-\infty$ \\[7pt]\hline
        
  \end{tabular}
  \caption{Conclusions for random walks based on LLN, LIL and CLT laws}\label{table:rw_laws}
\end{table*}

\subsection{Arcsine distribution: cdf and pdf}

\begin{figure}[ht]
 \centering
 %[width=\columnwidth]
 \includegraphics[scale=0.4]{figures2/arcsine_dist_5x8.pdf}
 \caption{Arcsine distribution.}
 \label{fig:asine_dist}
\end{figure}
\medskip\par\noindent


\subsection{experiments}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% RANDU %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{RANDU}
Let us start with an example of PRNG designed in the early 1960s which is no longer used.
RANDU was mentioned in Section \ref{subsec:prng} as an example of a generator definitely failing the spectral
test. This generator is defined as $MCG(2^{31}, 65539)$. Selecting $65539$ as the multiplicative constant seemed
to be good as $65539 = 2^{16} + 3$ what allows for performing fast multiplication on hardware.

The results of testing RANDU are shown in Tables \ref{tab:randu_asin} and \ref{tab:randu_lil}.
\begin{table*}[t!]
\centering
 \caption{Results of arcsine test for RANDU generator.}
 \label{tab:randu_asin}
\begin{tabular} {||c|c|c|c|c|c|c||}  
 \hline 
     n &  $2^{21}$ &  $2^{22}$ &  $2^{23}$ &  $2^{24}$ &  $2^{25}$ &  $2^{26}$\\ \hline
     tv &  0.4604 &  0.4616 &  0.4637 &  0.4670 &  0.4695 &  0.4697\\ \hline
   sep1 &  0.6017 &  0.6646 &  0.6229 &  0.6138 &  0.5934 &  0.6453\\ \hline
   sep2 &  0.8659 &  0.8662 &  0.8667 &  0.8675 &  0.8681 &  0.8682\\ \hline
  p-val &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline
\end{tabular}  
\end{table*}

\begin{table*}[t!]
\centering
 \caption{Results of LIL test for RANDU generator.}
 \label{tab:randu_lil}
\begin{tabular} {||c|c|c|c|c|c|c||}  
 \hline 
     n &  $2^{21}$ &  $2^{22}$ &  $2^{23}$ &  $2^{24}$ &  $2^{25}$ &  $2^{26}$\\ \hline
     tv &  0.4955 &   0.496 &  0.4965 &  0.4969 &  0.4973 &  0.4977\\ \hline
   sep1 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
   sep2 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
  p-val &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline
\end{tabular}  
\end{table*}

As we can observe, there is no need to generate very long sequences of pseudorandom bits to observe that the output
of RANDU is far from truly random. This explains why this PRNG was quickly superseded by other algorithms.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Borland C / C++ rand() %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Borland C/C++ rand()}
Procedure \texttt{rand} from standard library in Borland C/C++ implements $LCG(2^{32}, 22695477, 1)$.
Similarly to \texttt{rand} in MS Visual C++, it returns only the bits on positions 30..16.
Like in previous example in experiments we only use 8 most significant bits of numbers returned by tested PRNG.
\begin{table*}[t!]
\centering
 \caption{Results of arcsine test for PRNG in Borland C/C++ standard library.}
 \label{tab:borland_asin}
\begin{tabular} {||c|c|c|c|c|c|c|c|c|c|c|c||}  
 \hline
     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
     tv &  0.0384 &  0.0502 &  0.0697 &  0.0861 &  0.1394 &  0.1562 &  0.1231 &  0.1466 &  0.2148\\ \hline
   sep1 &  0.1293 &  0.1840 &  0.2513 &  0.3733 &  0.5485 &  0.5149 &  0.5696 &  0.6873 &  0.8219\\ \hline
   sep2 &  0.2024 &  0.2120 &  0.2096 &  0.3137 &  0.3702 &  0.3730 &  0.3799 &  0.5167 &  0.4009\\ \hline
  p-val &  0.0001 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline
\end{tabular}  
\end{table*}

\begin{table*}[t!]
\centering
 \caption{Results of LIL test for PRNG in Borland C/C++ standard library.}
 \label{tab:borland_lil}
\begin{tabular} {||c|c|c|c|c|c|c|c|c|c|c|c||}  
 \hline 
     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
     tv &  0.0684 &  0.1002 &  0.1395 &  0.1940 &  0.3187 &  0.4136 &  0.4685 &  0.5911 &  0.9500\\ \hline
   sep1 &  0.6752 &  0.7357 &  0.9193 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
   sep2 &  0.1610 &  0.2565 &  0.2978 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
  p-val &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline
\end{tabular}  
\end{table*}
Tables \ref{tab:borland_asin} and \ref{tab:borland_lil} contain the outcomes of experiments carried out
for Borland C/C++ stdlib \texttt{rand}. They are very akin to those for standard PRNG in MS Visual C++
and the same remarks as in Section \ref{subsec:expMSVisual} apply.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% CMRG %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{CMRG}
\label{subsec:CMRG}
CMRG, which stands for \emph{combined multiple recursive generator}, is one of so called combined generators,
discussed in paragraph \ref{subsec:prng}. This PRNG returns numbers from $Z_n$ computed according to the following formula
\begin{align}
    Z_n &= X_n - Y_n \mod 2^{31}-1 \nonumber \\
    X_n &= 63308 X_{n-2} - 183326 X_{n-3} \mod 2^{31}-1 \\
    \begin{split} Y_n &= 86098 Y_{n-1} - 539608 Y_{n-3} \\ & \quad \mod 2^{31} - 2000169 \end{split} \nonumber
\end{align}
In our tests we used bits 15..8 of the number $Z_n$ outputted by the generator. Experimental results obtained for CMRG
are gathered in Tables \ref{tab:cmrg_asin} and \ref{tab:cmrg_lil}.

\begin{table*}[t!]
\centering
 \caption{Results of arcsine test for CMRG.}
 \label{tab:cmrg_asin}
\begin{tabular} {||c|c|c|c|c|c|c|c|c|c|c|c||}  
 \hline
     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
     tv &  0.0191 &  0.0234 &  0.0235 &  0.0239 &  0.0232 &  0.0228 &  0.0218 &  0.0268 &  0.0272\\ \hline
   sep1 &  0.1135 &  0.2090 &  0.1187 &  0.1450 &  0.1607 &  0.1191 &  0.1232 &  0.1592 &  0.2084\\ \hline
   sep2 &  0.1402 &  0.0900 &  0.1084 &  0.1477 &  0.1934 &  0.1666 &  0.0931 &  0.1353 &  0.1158\\ \hline
  p-val &  0.9752 &  0.4101 &  0.8062 &  0.7402 &  0.4043 &  0.6841 &  0.9821 &  0.2394 &  0.1343\\ \hline
\end{tabular}  
\end{table*}

\begin{table*}[t!]
\centering
 \caption{Results of LIL test for CMRG.}
 \label{tab:cmrg_lil}
\begin{tabular} {||c|c|c|c|c|c|c|c|c|c|c|c||}  
 \hline 
     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
     tv &  0.0218 &  0.0241 &  0.0272 &  0.0203 &  0.0231 &  0.0251 &  0.0330 &  0.0233 &  0.0234\\ \hline
   sep1 &  0.2336 &  0.3273 &  0.1803 &  0.2551 &  0.3085 &  0.1690 &  0.3146 &  0.3310 &  0.2829\\ \hline
   sep2 &  0.3450 &  0.2105 &  0.1234 &  0.1032 &  0.1901 &  0.1658 &  0.2302 &  0.2486 &  0.1761\\ \hline
  p-val &  0.6046 &  0.2689 &  0.2030 &  0.8653 &  0.4581 &  0.3966 &  0.0128 &  0.4106 &  0.6803\\ \hline
\end{tabular}  
\end{table*}

At first glance we can see that this PRNG has rather long period and testing results give no reason for rejecting
the hypothesis about the randomness of bit sequences produces by this PRNG. Nevertheless, one should note that in \cite{Kim2008} 
the authors provide strong evidence that the output of CMRG is not sound.

==> sections/tables_figures.tex <==
\begin{table*}
  \centering%
  \begin{tabular}{|l|l|l|l|l|}\hline
   & conv. in prob. & a.s. conv. & $\limsup$ a.s & $\liminf$ a.s \\[7pt]\hline
    LLN & ${S_n\over n}\stackrel{P}{\to}0$ & ${S_n\over n}\stackrel{a.s.}{\to}0$
    & $\displaystyle\limsup_{n\to\infty} {S_n\over n}=0$ & $\displaystyle\liminf_{n\to\infty}{S_n\over n}=0$ \\[7pt]\hline
    
    LIL & ${S_n\over 2n\log\log n}\stackrel{P}{\to}0$ & ${S_n\over 2n\log \log n}\stackrel{a.s.}{\nrightarrow }0$
    & $\displaystyle\limsup_{n\to\infty} {S_n\over 2n\log\log n}=1$ & $\displaystyle\liminf_{n\to\infty}{S_n\over 2n\log\log n}=-1$ \\[17pt]\hline
    
    
    CLT & $\forall x {S_n\over n}\stackrel{P}{\nrightarrow}x$ & $\forall x {S_n\over n}\stackrel{a.s.}{\nrightarrow }x$
    & $\displaystyle\limsup_{n\to\infty} {S_n \over n}=\infty$ & $\displaystyle\liminf_{n\to\infty}{S_n\over n}=-\infty$ \\[7pt]\hline
        
  \end{tabular}
  \caption{Conclusions for random walks based on LLN, LIL and CLT laws}\label{table:rw_laws}
\end{table*}


\begin{figure}
\centering
%[width=\columnwidth]
\includegraphics[scale=0.4]{figures/trajectories_6x8.pdf}
\caption{500 trajectories of random walks of length $2^{30}$. Blue plot: $\pm \sqrt{n}$, red plot: $\pm \sqrt{2n\log\log n}$ }\label{fig:500iter}
\end{figure}

\begin{figure}[ht]
 \centering
 %[width=\columnwidth]
 \includegraphics[scale=0.4]{figures/arcsine_dist_5x8.pdf}
 \caption{Arcsine distribution.}
 \label{fig:asine_dist}
\end{figure}

\begin{table*}[t!]
\centering
 \caption{Results of arcsine test for RANDU generator.}
 \label{tab:randu_asin}
\begin{tabular} {||c|c|c|c|c|c|c||}  
 \hline 
     n &  $2^{21}$ &  $2^{22}$ &  $2^{23}$ &  $2^{24}$ &  $2^{25}$ &  $2^{26}$\\ \hline
     tv &  0.4604 &  0.4616 &  0.4637 &  0.4670 &  0.4695 &  0.4697\\ \hline
   sep1 &  0.6017 &  0.6646 &  0.6229 &  0.6138 &  0.5934 &  0.6453\\ \hline
   sep2 &  0.8659 &  0.8662 &  0.8667 &  0.8675 &  0.8681 &  0.8682\\ \hline
  p-val &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline
\end{tabular}  
\end{table*}

\begin{table*}[t!]
\centering
 \caption{Results of LIL test for RANDU generator.}
 \label{tab:randu_lil}
\begin{tabular} {||c|c|c|c|c|c|c||}  
 \hline 
     n &  $2^{21}$ &  $2^{22}$ &  $2^{23}$ &  $2^{24}$ &  $2^{25}$ &  $2^{26}$\\ \hline
     tv &  0.4955 &   0.496 &  0.4965 &  0.4969 &  0.4973 &  0.4977\\ \hline
   sep1 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
   sep2 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
  p-val &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline
\end{tabular}  
\end{table*}

\begin{table*}[t!]
\centering
 \caption{Results of arcsine test for PRNG in MS Visual C++.}
 \label{tab:svis_asin}
\begin{tabular} {||c|c|c|c|c|c|c|c|c|c|c|c||}  
 \hline
     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
     tv &  0.0289 &  0.0387 &  0.0615 &  0.0768 &  0.0848 &  0.0928 &  0.0965 &  0.1870 &  0.2093\\ \hline
   sep1 &  0.2030 &  0.1548 &  0.1952 &  0.2605 &  0.3664 &  0.4210 &  0.5528 &  0.6533 &  0.8163\\ \hline
   sep2 &  0.1780 &  0.2260 &  0.2524 &  0.2364 &  0.2841 &  0.3160 &  0.4336 &  0.6112 &  0.4328\\ \hline
  p-val &  0.0128 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline 
\end{tabular}  
\end{table*}

\begin{table*}[t!]
\centering
 \caption{Results of LIL test for PRNG in MS Visual C++.}
 \label{tab:svis_lil}
\begin{tabular} {||c|c|c|c|c|c|c|c|c|c|c|c||}  
 \hline 
     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
     tv &  0.0350 &  0.0512 &  0.0938 &  0.1234 &  0.1672 &  0.2423 &  0.3100 &  0.4991 &  0.9500\\ \hline
   sep1 &  0.2831 &  0.7419 &  0.9731 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
   sep2 &  0.2670 &  0.1416 &  0.2635 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
  p-val &  0.0001 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline
\end{tabular}  
\end{table*}



\begin{table*}[t!]
\centering
 \caption{Results of arcsine test for PRNG in Borland C/C++ standard library.}
 \label{tab:borland_asin}
\begin{tabular} {||c|c|c|c|c|c|c|c|c|c|c|c||}  
 \hline
     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
     tv &  0.0384 &  0.0502 &  0.0697 &  0.0861 &  0.1394 &  0.1562 &  0.1231 &  0.1466 &  0.2148\\ \hline
   sep1 &  0.1293 &  0.1840 &  0.2513 &  0.3733 &  0.5485 &  0.5149 &  0.5696 &  0.6873 &  0.8219\\ \hline
   sep2 &  0.2024 &  0.2120 &  0.2096 &  0.3137 &  0.3702 &  0.3730 &  0.3799 &  0.5167 &  0.4009\\ \hline
  p-val &  0.0001 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline
\end{tabular}  
\end{table*}

\begin{table*}[t!]
\centering
 \caption{Results of LIL test for PRNG in Borland C/C++ standard library.}
 \label{tab:borland_lil}
\begin{tabular} {||c|c|c|c|c|c|c|c|c|c|c|c||}  
 \hline 
     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
     tv &  0.0684 &  0.1002 &  0.1395 &  0.1940 &  0.3187 &  0.4136 &  0.4685 &  0.5911 &  0.9500\\ \hline
   sep1 &  0.6752 &  0.7357 &  0.9193 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
   sep2 &  0.1610 &  0.2565 &  0.2978 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
  p-val &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline
\end{tabular}  
\end{table*}




\begin{table*}[t!]
\centering
 \caption{Results of arcsine test for initial version of PRNG from BSD libc.}
 \label{tab:bsd_asin}
\begin{tabular} {||c|c|c|c|c|c|c||}  
 \hline 
      n &  $2^{21}$ &  $2^{22}$ &  $2^{23}$ &  $2^{24}$ &  $2^{25}$ &  $2^{26}$\\ \hline
     tv &  0.0883 &  0.0980 &  0.0862 &  0.0951 &  0.0936 &  0.1081\\ \hline
   sep1 &  0.3402 &  0.3979 &  0.4111 &  0.4980 &  0.4346 &  0.4751\\ \hline
   sep2 &  0.3634 &  0.4198 &  0.3053 &  0.2805 &  0.3424 &  0.4070\\ \hline
  p-val &  0.1829 &  0.0326 &  0.1874 &  0.1767 &  0.1181 &  0.0051\\ \hline
\end{tabular}  
\end{table*}

\begin{table*}[t!]
\centering
 \caption{Results of LIL test for initial version of PRNG from BSD libc.}
 \label{tab:bsd_lil}
\begin{tabular} {||c|c|c|c|c|c|c||}  
 \hline 
      n &  $2^{21}$ &  $2^{22}$ &  $2^{23}$ &  $2^{24}$ &  $2^{25}$ &  $2^{26}$\\ \hline
     tv &  0.1956 &  0.2191 &  0.2472 &  0.2539 &  0.2464 &  0.2707\\ \hline
   sep1 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
   sep2 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
  p-val &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline
\end{tabular}  
\end{table*}

\begin{table*}[t!]
\centering
 \caption{Results of arcsine test for GNU C standard library generator.}
 \label{tab:mojkomp_asin}
\begin{tabular} {||c|c|c|c|c|c|c|c|c|c|c|c||}  
 \hline
     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
     tv &  0.0287 &  0.0217 &  0.0264 &  0.0228 &  0.0202 &  0.0289 &  0.0237 &  0.0254 &  0.0230\\ \hline
   sep1 &  0.1157 &  0.1249 &  0.1629 &  0.1186 &  0.1661 &  0.1717 &  0.1306 &  0.1316 &  0.1405\\ \hline
   sep2 &  0.1754 &  0.1909 &  0.1436 &  0.1869 &  0.1110 &  0.1344 &  0.1786 &  0.1262 &  0.1879\\ \hline
  p-val &  0.0649 &  0.5511 &  0.2565 &  0.4887 &  0.7967 &  0.1115 &  0.5880 &  0.2599 &  0.3930\\ \hline 
\end{tabular}  
\end{table*}

\begin{table*}[t!]
\centering
 \caption{Results of LIL test for GNU C standard library generator.}
 \label{tab:mojkomp_lil}
\begin{tabular} {||c|c|c|c|c|c|c|c|c|c|c|c||}  
 \hline 
     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
     tv &  0.0185 &  0.0243 &  0.0242 &  0.0244 &  0.0210 &  0.0220 &  0.0330 &  0.0237 &  0.0221\\ \hline
   sep1 &  0.2593 &  0.1640 &  0.1844 &  0.2573 &  0.2010 &  0.1853 &  0.2882 &  0.4129 &  0.2563\\ \hline
   sep2 &  0.0807 &  0.2133 &  0.2299 &  0.2060 &  0.1839 &  0.2361 &  0.3456 &  0.2078 &  0.1405\\ \hline
  p-val &  0.9627 &  0.4878 &  0.5225 &  0.3022 &  0.6978 &  0.5382 &  0.0009 &  0.4903 &  0.7901\\ \hline
\end{tabular}  
\end{table*}

\begin{table*}[t!]
\centering
 \caption{Results of arcsine test for Minstd generator with multiplier 16807.}
 \label{tab:minstd_asin}
\begin{tabular} {||c|c|c|c|c|c|c|c|c|c|c|c||}  
 \hline
     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
     tv &  0.0321 &  0.0321 &  0.0402 &  0.0725 &  0.0917 &  0.1116 &  0.1648 &  0.2003 &  0.2109\\ \hline
   sep1 &  0.1172 &  0.1686 &  0.1407 &  0.2985 &  0.2880 &  0.6670 &  0.5203 &  0.7345 &  0.8486\\ \hline
   sep2 &  0.1302 &  0.1490 &  0.2420 &  0.3986 &  0.4051 &  0.3735 &  0.3822 &  0.5352 &  0.3894\\ \hline
  p-val &  0.0360 &  0.0203 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline
\end{tabular}  
\end{table*}

\begin{table*}[t!]
\centering
 \caption{Results of LIL test for Minstd generator with multiplier 16807.}
 \label{tab:minstd_lil}
\begin{tabular} {||c|c|c|c|c|c|c|c|c|c|c|c||}  
 \hline 
     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
     tv &  0.0370 &  0.0622 &  0.0823 &  0.1120 &  0.1877 &  0.2002 &  0.3538 &  0.3194 &  0.9500\\ \hline
   sep1 &  0.5035 &  0.5465 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
   sep2 &  0.1444 &  0.2366 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
  p-val &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline
\end{tabular}  
\end{table*}


\begin{table*}[t!]
\centering
 \caption{Results of arcsine test for Minstd generator with multiplier 48271.}
 \label{tab:nminstd_asin}
\begin{tabular} {||c|c|c|c|c|c|c|c|c|c|c|c||}  
 \hline
     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
     tv &  0.0318 &  0.0430 &  0.0477 &  0.0982 &  0.1303 &  0.0918 &  0.0848 &  0.1131 &  0.2089\\ \hline
   sep1 &  0.1607 &  0.1467 &  0.1901 &  0.3803 &  0.4280 &  0.3845 &  0.4583 &  0.3975 &  0.8079\\ \hline
   sep2 &  0.1828 &  0.1719 &  0.2120 &  0.2548 &  0.3449 &  0.3179 &  0.3192 &  0.3186 &  0.4579\\ \hline
  p-val &  0.0115 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline
\end{tabular}  
\end{table*}

\begin{table*}[t!]
\centering
 \caption{Results of LIL test for Minstd generator with multiplier 48271.}
 \label{tab:nminstd_lil}
\begin{tabular} {||c|c|c|c|c|c|c|c|c|c|c|c||}  
 \hline 
     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
     tv &  0.0372 &  0.0563 &  0.0590 &  0.2573 &  0.2879 &  0.3408 &  0.3167 &  0.3434 &  0.9500\\ \hline
   sep1 &  0.3298 &  0.4839 &  0.9328 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
   sep2 &  0.3843 &  0.1850 &  0.2207 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000 &  1.0000\\ \hline
  p-val &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline
\end{tabular}  
\end{table*}



\begin{table*}[t!]
\centering
 \caption{Results of arcsine test for CMRG.}
 \label{tab:cmrg_asin}
\begin{tabular} {||c|c|c|c|c|c|c|c|c|c|c|c||}  
 \hline
     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
     tv &  0.0191 &  0.0234 &  0.0235 &  0.0239 &  0.0232 &  0.0228 &  0.0218 &  0.0268 &  0.0272\\ \hline
   sep1 &  0.1135 &  0.2090 &  0.1187 &  0.1450 &  0.1607 &  0.1191 &  0.1232 &  0.1592 &  0.2084\\ \hline
   sep2 &  0.1402 &  0.0900 &  0.1084 &  0.1477 &  0.1934 &  0.1666 &  0.0931 &  0.1353 &  0.1158\\ \hline
  p-val &  0.9752 &  0.4101 &  0.8062 &  0.7402 &  0.4043 &  0.6841 &  0.9821 &  0.2394 &  0.1343\\ \hline
\end{tabular}  
\end{table*}

\begin{table*}[t!]
\centering
 \caption{Results of LIL test for CMRG.}
 \label{tab:cmrg_lil}
\begin{tabular} {||c|c|c|c|c|c|c|c|c|c|c|c||}  
 \hline 
     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
     tv &  0.0218 &  0.0241 &  0.0272 &  0.0203 &  0.0231 &  0.0251 &  0.0330 &  0.0233 &  0.0234\\ \hline
   sep1 &  0.2336 &  0.3273 &  0.1803 &  0.2551 &  0.3085 &  0.1690 &  0.3146 &  0.3310 &  0.2829\\ \hline
   sep2 &  0.3450 &  0.2105 &  0.1234 &  0.1032 &  0.1901 &  0.1658 &  0.2302 &  0.2486 &  0.1761\\ \hline
  p-val &  0.6046 &  0.2689 &  0.2030 &  0.8653 &  0.4581 &  0.3966 &  0.0128 &  0.4106 &  0.6803\\ \hline
\end{tabular}  
\end{table*}


\begin{table*}[t!]
\centering
 \caption{Results of arcsine test for C++11 implementation of MT19937-64 generator.}
 \label{tab:twister_asin}
\begin{tabular} {||c|c|c|c|c|c|c|c|c|c|c|c||}  
 \hline
     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
     tv &  0.0271 &  0.0245 &  0.0226 &  0.0281 &  0.0276 &  0.0228 &  0.0271 &  0.0230 &  0.0255\\ \hline
   sep1 &  0.1421 &  0.1606 &  0.1167 &  0.1824 &  0.1938 &  0.1571 &  0.1760 &  0.1397 &  0.1573\\ \hline
   sep2 &  0.1133 &  0.1195 &  0.1056 &  0.1399 &  0.1256 &  0.1287 &  0.1391 &  0.0994 &  0.1444\\ \hline
  p-val &  0.2755 &  0.6823 &  0.8804 &  0.0801 &  0.1267 &  0.7343 &  0.1094 &  0.7596 &  0.2029\\ \hline
\end{tabular}  
\end{table*}

\begin{table*}[t!]
\centering
 \caption{Results of LIL test for C++11 implementation of MT19937-64 generator.}
 \label{tab:twister_lil}
\begin{tabular} {||c|c|c|c|c|c|c|c|c|c|c|c||}  
 \hline 
     n &  $2^{26}$ &  $2^{27}$ &  $2^{28}$ &  $2^{29}$ &  $2^{30}$ &  $2^{31}$ &  $2^{32}$ &  $2^{33}$ &  $2^{34}$\\ \hline
     tv &  0.0254 &  0.0264 &  0.0238 &  0.0234 &  0.0266 &  0.0265 &  0.0290 &  0.0299 &  0.0215\\ \hline
   sep1 &  0.1853 &  0.2147 &  0.1689 &  0.3093 &  0.1887 &  0.2015 &  0.2877 &  0.2318 &  0.1953\\ \hline
   sep2 &  0.2841 &  0.1696 &  0.1917 &  0.1282 &  0.2017 &  0.2492 &  0.1842 &  0.1541 &  0.1716\\ \hline
  p-val &  0.2483 &  0.3690 &  0.5965 &  0.5066 &  0.2196 &  0.1495 &  0.0499 &  0.0189 &  0.8170\\ \hline
\end{tabular}  
\end{table*}


\begin{table*}[t!]
\centering
 \caption{Results of arcsine test for the flawed generator described in Section \ref{subsec:experiments_flawed}.}
 \label{tab:zep_asin}
\begin{tabular} {||c|c|c|c|c|c|c|c|c|c|c|c||}  
 \hline
     n  &  $2^{20}$ &  $2^{21}$ &  $2^{22}$ &  $2^{23}$ &  $2^{24}$ &  $2^{25}$ &  $2^{26}$ &  $2^{27}$ &  $2^{28}$\\ \hline
     tv &  0.0326 &  0.0241 &  0.0281 &  0.0285 &  0.0298 &  0.0339 &  0.0298 &  0.0285 &  0.0276\\ \hline
   sep1 &  0.1466 &  0.1754 &  0.1529 &  0.1124 &  0.1249 &  0.1752 &  0.1594 &  0.1666 &  0.1257\\ \hline
   sep2 &  0.3255 &   0.334 &   0.345 &  0.4212 &  0.3608 &  0.3582 &  0.3556 &  0.3925 &  0.3901\\ \hline
  p-val &  0.0000 &  0.0031 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000 &  0.0000\\ \hline
\end{tabular}  
\end{table*}

\begin{table*}[t!]
\centering
 \caption{Results of LIL test for the flawed generator described in Section \ref{subsec:experiments_flawed}.}
 \label{tab:zep_lil}
\begin{tabular} {||c|c|c|c|c|c|c|c|c|c|c|c||}  
 \hline 
     n  &  $2^{20}$ &  $2^{21}$ &  $2^{22}$ &  $2^{23}$ &  $2^{24}$ &  $2^{25}$ &  $2^{26}$ &  $2^{27}$ &  $2^{28}$\\ \hline
     tv &  0.0239 &  0.0303 &  0.0255 &  0.0269 &  0.0241 &  0.0280 &  0.0248 &  0.0294 &  0.0229\\ \hline
   sep1 &  0.1929 &  0.2834 &  0.1541 &  0.2018 &  0.2327 &  0.1586 &  0.1631 &  0.2654 &  0.1689\\ \hline
   sep2 &  0.1625 &  0.1517 &  0.1663 &  0.1469 &  0.1381 &  0.1648 &  0.2106 &  0.1667 &  0.1815\\ \hline
  p-val &  0.4073 &  0.0199 &  0.2584 &  0.1250 &  0.5742 &  0.1250 &  0.2703 &  0.0436 &  0.5789\\ \hline
\end{tabular}  
\end{table*}


